A Unified Framework for Tuning Hyperparameters in Clustering Problems

Selecting hyperparameters for unsupervised learning problems is challenging in general due to the lack of ground truth for validation. Despite the prevalence of this issue in statistics and machine learning, especially in clustering problems, there are not many methods for tuning these hyperparameters with theoretical guarantees. In this paper, we provide a framework with provable guarantees for selecting hyperparameters in a number of distinct models. We consider both the subgaussian mixture model and network models to serve as examples of i.i.d. and non-i.i.d. data. We demonstrate that the same framework can be used to choose the Lagrange multipliers of penalty terms in semi-definite programming (SDP) relaxations for community detection, and the bandwidth parameter for constructing kernel similarity matrices for spectral clustering. By incorporating a cross-validation procedure, we show the framework can also do consistent model selection for network models. Using a variety of simulated and real data examples, we show that our framework outperforms other widely used tuning procedures in a broad range of parameter settings.

==> latexmkrc.tex <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );
 
        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );
 
        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
 
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> sec_mmsb.tex <==
\section{Model selection for MMSB}
\label{sec:mmsb}
Similar to the proof of SBM, 

First, we show for any underestimated normalized clustering matrix, i.e., $\text{trace}(\hat{X})< r_0$, if it is independent of $A$, then with high probability, $\langle A, \hat{X} \rangle \leq \langle A, X_0 \rangle - \Omega(np_{\text{gap}}\pi_\text{min}^2/r^2)$.


==> supp_arxiv.tex <==
\clearpage
\section*{}
\begin{center}
{\large\bf SUPPLEMENTARY MATERIAL}
\end{center}
\appendix
This appendix contains detailed proofs of theoretical results in the main paper  ``A Unified Framework for Tuning Hyperparameters in Clustering Problems'', additional theoretical results, and detailed description of the experimental parameter settings. 
We present proofs for MATR and MATR-CV in Sections~\ref{sec:proofformatr} and Sections~\ref{sec:proofformatrcv} respectively. Sections~\ref{sec:merge1} and~\ref{sec:merge2} also contain additional theoretical results on the role of the hyperparameter in merging clusters in~\ref{SDP:YD} and~\ref{SDP:BW} respectively.
Finally, Section~\ref{sec:expdetail} contains detailed parameter settings for the experimental results in the main paper.

\section{Additional theoretical results and proofs of results in Section~\ref{sec:knownk}}\label{sec:proofformatr}
\subsection{Proof of Theorem \ref{thm:general_setup}}
\label{sec:thm1}
\iffalse
\begin{proof}
If for tuning parameter $\lambda$, we have $\langle \hat{S}, \hat{X}_{\lambda} \rangle \geq \langle S, X_0 \rangle -\epsilon$, then 
	\begin{align}
	    \langle S, \hat{X}_{\lambda} \rangle \geq \langle S, X_0 \rangle - |\langle \hat{S} - S, \hat{X}_{\lambda} \rangle|- \epsilon.
	\end{align} 	
	First we will prove that this immediately gives an upper bound on $\|\hat{X}_\lambda-X_0\|_F$.
	We will remove the subscript $\lambda$ for ease of exposition.
	Denote $\omega_k=\langle X_0, \hat{X}_{S_k, S_k}\rangle$, $\alpha_{kl} = \frac{\langle E_{S_k, S_l}, \hat{X}\rangle}{m_k(1-\omega_k)},$ when $\omega_k<1$ and $0$ otherwise. Then we have 
	\begin{equation}
	\begin{split}
	\langle S, \hat{X} \rangle &=\sum_k a_{kk} \langle E_{S_k, S_k}, \hat{X} \rangle + \sum_{k\neq l} a_{kl} \langle E_{S_k,S_l}, 
	\hat{X} \rangle\\
	&=\sum_k a_{kk} m_k \omega_k + \sum_k m_k (1-\omega_k) \sum_{l\neq k} a_{kl} \alpha_{kl}\\
	&=\sum_k m_k \omega_k(a_{kk}-\sum_{l\neq k} a_{kl}\alpha_{kl}) + \sum_k m_k \sum_{l\neq k} a_{kl} \alpha_{kl}
	\end{split}
	\end{equation}
	
	Since by assumption $\langle S, \hat{X} \rangle \geq \sum_k m_k a_{kk} -|\langle R, \hat{X} \rangle|- \epsilon$, 
	$$\sum_k m_k \omega_k(a_{kk}-\sum_{l\neq k} a_{kl}\alpha_{kl}) + \sum_k m_k \sum_{l\neq k} a_{kl} \alpha_{kl} \geq \sum_k m_k a_{kk} -|\langle R, \hat{X} \rangle|- \epsilon.$$
	
	Note that, since $S$ is weakly assortative, $a_{kk}-\sum a_{kl}\alpha_{kl}$ is always positive because $\sum_{l\neq k} \alpha_{kl} \leq 1$.
	
	Denote $\epsilon' =|\langle R, \hat{X} \rangle|+\epsilon $, $\beta_k = \frac{m_k (a_{kk}- \sum_{l\neq k} \alpha_{kl}a_{kl})}{\sum_k m_k (a_{kk} - \sum_{l\neq k} \alpha_{kl}a_{kl})}$,
	\begin{align*}
	   \sum_k m_k \omega_k(a_{kk}-\sum_{l\neq k} a_{kl}\alpha_{kl})&\geq \sum_k m_k (a_{kk} - \sum_{l\neq k} \alpha_{kl}a_{kl}) -\epsilon'\\
	   \sum_k \beta_k \omega_k&\geq 1 -\frac{\epsilon'}{ \sum_k m_k (a_{kk} - \sum_{l\neq k} \alpha_{kl}a_{kl}) }\\
	   \sum_k \beta_k (1-\omega_k) &\leq \frac{\epsilon'}{ \sum_k m_k (a_{kk} - \sum_{l\neq k} \alpha_{kl}a_{kl}) }.\\
	   \sum_k (1-\omega_k) &\leq \sum_k \frac{\beta_k}{\beta_{\min}} (1-\omega_k)\leq \frac{\epsilon'}{ \beta_{\min}\sum_k m_k (a_{kk} - \sum_{l\neq k} \alpha_{kl}a_{kl}) },
	\end{align*}
	where $\beta_{\min}=\min_k\beta_k$.
%	$$\$$
%	$$\sum_k \beta_k T_k\geq 1 -\frac{\epsilon ^*}{ \sum_k m_k (a_{kk} - \sum_{l\neq k} \alpha_{kl}a_{kl}) },$$
%	$$\sum_k \beta_k (1-T_k) \leq \frac{\epsilon ^*}{ \sum_k m_k (a_{kk} - \sum_{l\neq k} \alpha_{kl}a_{kl}) }.$$
	Since $\text{trace}(\hat{X}) = \text{trace}(X_0)$,
	\begin{equation}
	\begin{aligned}
	\norm{\hat{X} - X_0}_F^2 &= \text{trace}((\hat{X}-X_0)^T(\hat{X}-X_0))\nonumber\\
	&= \text{trace}(\hat{X}+X_0 - 2\hat{X}X_0)\nonumber\\
	&= 2\text{trace}(X_0) - 2\sum_{k}\langle X_0,\hat{X}_{S_k,S_k}\rangle\nonumber\\
	&= 2 \sum_k(1-\omega_k)\leq \frac{2\epsilon'}{\min_k {m_k (a_{kk} - \sum_{l\neq k}   \alpha_{kl}a_{kl})}}\nonumber  \\
	&\leq  \frac{2\epsilon'}{n\pi_{\min}\min_k (a_{kk} - \max_{l\neq k}   a_{kl})}  \label{eq:normub}
	\end{aligned}
	\end{equation}
% 	If Algorithm $\mathscr{A}$ outputs a $\hat{Z}_{\lambda_*}$, and for the corresponding normalized clustering matrix  $\hat{X}_{\lambda_*}$  Eq~\ref{eq:assump} holds, then 
% 	if $\lambda_0$ is in the range of tuning parameters considered by Algorithm~\ref{alg:kk}, we know that for the $\lambda_*$ returned by MATR, 
	Now consider the $\lambda_*$ returned by MATR, 
%	\begin{align*}
% 	\begin{align*}
% 	\langle \hat{S}, \hat{X}_{\lambda_*} \rangle \geq \langle \hat{S}, \hat{X}_{\lambda_0} \rangle &\geq \langle S, X_0 \rangle - |\langle \hat{S} - S, \hat{X}_{\lambda_0} \rangle|- \epsilon\\
% 	&\geq \langle S, X_0 \rangle-\underbrace{\sup_{X\in \mathcal{X}_r}|\langle X, R\rangle|-\epsilon}_{\epsilon_*}
% 	\end{align*}
	
	$$	\langle \hat{S}, \hat{X}_{\lambda_*} \rangle \geq \langle \hat{S}, \hat{X}_{\lambda_0} \rangle \geq \langle S, X_0 \rangle - \epsilon.$$
	
	Then, following the above argument and from the condition from the theorem, 
	$$\|X_{\lambda_*}-X_0\|_F^2\leq \frac{2\epsilon'}{n\pi_{\min}\min_k (a_{kk} - \max_{l\neq k}   a_{kl})}=o_P(1).$$
	
\end{proof}
\fi

\begin{proof}
If for tuning parameter $\lambda$, we have $\langle \hat{S}, \hat{X}_{\lambda} \rangle \geq \langle S, X_0 \rangle -\epsilon$, then 
	\begin{align}\label{eq:assump}
	    \langle S, \hat{X}_{\lambda} \rangle \geq \langle S, X_0 \rangle - |\langle \hat{S} - S, \hat{X}_{\lambda} \rangle|- \epsilon.
	\end{align} 	
	First we will prove that this immediately gives an upper bound on $\|\hat{X}_\lambda-X_0\|_F$.
	We will remove the subscript $\lambda$ for ease of exposition.
	Denote $\omega_k=\langle X_0, \hat{X}_{C_k, C_k}\rangle$, $\alpha_{ij} = \frac{\langle E_{i, j}, \hat{X}\rangle}{m_k(1-\omega_k)},$ when $\omega_k<1$ and $0$ otherwise, and off-diagonal set for $k$th cluster $C_{k}^c$ as $\{(i,j)|i\in C_k, j\notin C_k\}$. Then we have 
	\begin{equation}
	\begin{split}
	\langle S, \hat{X} \rangle &=\sum_{k=1}^{r_0} a_{kk} \langle E_{C_k, C_k}, \hat{X} \rangle + \sum_{k=1}^{r_0}\sum_{(i,j)\in C_{k}^c} a_{ij} \langle E_{i,j}, 
	\hat{X} \rangle\\
	&=\sum_{k=1}^{r_0} a_{kk} m_k \omega_k + \sum_{k=1}^{r_0} m_k (1-\omega_k) \sum_{(i,j)\in C_{k}^c} a_{ij} \alpha_{ij}\\
	&=\sum_{k=1}^{r_0} m_k \omega_k(a_{kk}-\sum_{(i,j)\in C_{k}^c} a_{ij}\alpha_{ij}) + \sum_{k=1}^{r_0} m_k \sum_{(i,j)\in C_{k}^c} a_{ij} \alpha_{ij}
	\end{split}
	\end{equation}
	
	Since $\langle S, X_0\rangle=\sum_k m_k a_{kk}$, by~\eqref{eq:assump}, $\langle S, \hat{X} \rangle \geq \sum_k m_k a_{kk} -|\langle R, \hat{X} \rangle|- \epsilon$, we have
	$$\sum_k m_k \omega_k(a_{kk}-\sum_{(i,j)\in C_{k}^c} a_{ij}\alpha_{ij}) + \sum_k m_k \sum_{(i,j)\in C_{k}^c} a_{ij} \alpha_{ij} \geq \sum_k m_k a_{kk} -|\langle R, \hat{X} \rangle|- \epsilon.$$
	
	Note that, since $S$ is weakly assortative, $a_{kk}-\sum_{(i,j)\in C_{k}^c} a_{ij}\alpha_{ij}$ is always positive because $\sum_{(i,j)\in C_{k}^c} \alpha_{ij} \leq 1$.
	
	Denote $\epsilon' =|\langle R, \hat{X} \rangle|+\epsilon $, $\beta_k = \frac{m_k (a_{kk}- \sum_{C_{k}^c} \alpha_{ij}a_{ij})}{\sum_k m_k (a_{kk} - \sum_{C_{k}^c} \alpha_{ij}a_{ij})}$,
	\begin{align*}
	   \sum_k m_k \omega_k(a_{kk}-\sum_{(i,j)\in C_{k}^c} a_{ij}\alpha_{ij})&\geq \sum_k m_k (a_{kk} - \sum_{(i,j)\in C_{k}^c} \alpha_{ij}a_{ij}) -\epsilon'\\
	   \sum_k \beta_k \omega_k&\geq 1 -\frac{\epsilon'}{ \sum_k m_k (a_{kk} - \sum_{C_{k}^c} \alpha_{ij}a_{ij}) }\\
	   \sum_k \beta_k (1-\omega_k) &\leq \frac{\epsilon'}{ \sum_k m_k (a_{kk} - \sum_{C_{k}^c} \alpha_{ij}a_{ij}) }.\\
	   \sum_k (1-\omega_k) &\leq \sum_k \frac{\beta_k}{\beta_{\min}} (1-\omega_k)\leq \frac{\epsilon'}{ \beta_{\min}\sum_k m_k (a_{kk} - \sum_{C_{k}^c} \alpha_{ij}a_{ij}) },
	\end{align*}
	where $\beta_{\min}=\min_k\beta_k$.
%	$$\$$
%	$$\sum_k \beta_k T_k\geq 1 -\frac{\epsilon ^*}{ \sum_k m_k (a_{kk} - \sum_{l\neq k} \alpha_{kl}a_{kl}) },$$
%	$$\sum_k \beta_k (1-T_k) \leq \frac{\epsilon ^*}{ \sum_k m_k (a_{kk} - \sum_{l\neq k} \alpha_{kl}a_{kl}) }.$$
	Since $\text{trace}(\hat{X}) = \text{trace}(X_0)$,
	\begin{equation}
	\begin{aligned}
	\norm{\hat{X} - X_0}_F^2 &= \text{trace}((\hat{X}-X_0)^T(\hat{X}-X_0))\nonumber\\
	&= \text{trace}(\hat{X}+X_0 - 2\hat{X}X_0)\nonumber\\
	&= 2\text{trace}(X_0) - 2\sum_{k}\langle X_0,\hat{X}_{C_k,C_k}\rangle\nonumber\\
	&= 2 \sum_k(1-\omega_k)\leq \frac{2\epsilon'}{\min_k {m_k (a_{kk} - \sum_{C_{k}^c}   \alpha_{ij}a_{ij})}}\nonumber  \\
	&\leq  \frac{2\epsilon'}{n\pi_{\min}\min_k (a_{kk} - \max_{C_{k}^c}   a_{ij})} = \frac{2\epsilon'}{\tau}. \label{eq:normub}
	\end{aligned}
	\end{equation}
% 	If Algorithm $\mathscr{A}$ outputs a $\hat{Z}_{\lambda_*}$, and for the corresponding normalized clustering matrix  $\hat{X}_{\lambda_*}$  Eq~\ref{eq:assump} holds, then 
% 	if $\lambda_0$ is in the range of tuning parameters considered by Algorithm~\ref{alg:kk}, we know that for the $\lambda_*$ returned by MATR, 
	Now consider the $\lambda_*$ returned by MATR, 
%	\begin{align*}
% 	\begin{align*}
% 	\langle \hat{S}, \hat{X}_{\lambda_*} \rangle \geq \langle \hat{S}, \hat{X}_{\lambda_0} \rangle &\geq \langle S, X_0 \rangle - |\langle \hat{S} - S, \hat{X}_{\lambda_0} \rangle|- \epsilon\\
% 	&\geq \langle S, X_0 \rangle-\underbrace{\sup_{X\in \mathcal{X}_r}|\langle X, R\rangle|-\epsilon}_{\epsilon_*}
% 	\end{align*}
	
	$$	\langle \hat{S}, \hat{X}_{\lambda_*} \rangle \geq \langle \hat{S}, \hat{X}_{\lambda} \rangle \geq \langle S, X_0 \rangle - \epsilon.$$
	Then, following the above argument and from the condition from the theorem, 
	$$\|X_{\lambda_*}-X_0\|_F^2\leq \frac{2\epsilon'}{n\pi_{\min}\min_k (a_{kk} - \max_{C_{k}^c}   a_{ij})} \leq \frac{2}{\tau}(\epsilon+\sup_{X\in \mathcal{X}_{r_0}} |\langle X, R\rangle |).$$
	
\end{proof}

%\section{Proofs for \ref{SDP:YD}}
\subsection{Range of $\lambda$ for merging clusters in \ref{SDP:YD}}
\label{sec:merge1}
\begin{Proposition}\label{prop:sdp1merge}
	Let $\tilde{X}$ be the optimal solution of \ref{SDP:YD} for $A\sim SBM(B,Z_0)$ with $\lambda$ satisfying
	\begin{equation}
	\begin{split}
	\max_{k\neq \ell}B^*_{k,\ell} + \Omega(\sqrt{\frac{\rho \log n}{n\pi_\text{min}}})\leq\lambda  \leq \min_k B_{kk}^* -\max_{k, \ell=r-1,r} \frac{m_{\ell}}{n_k}(B_{\ell,\ell}-B_{r,r-1})+ O(\sqrt{\frac{\rho \log n}{n}}),
	\end{split}\nonumber
	\end{equation}
	then $\tilde{X}=X^*$ with probability at least $1-\frac{1}{n}$, where $X^*$ is the unnormalized clustering matrix which merges the last two clusters, $B^*$ is the  corresponding $(r-1)\times(r-1)$ block probability matrix. 
	% $X^*=Z^*\text{diag}(m^*)^{-1}Z^{*T}$, $Z^*=Z(I-E_{K,K}+E_{K,K-1})$($E_{i,j}$ is the matrix only with $E_{ij}=1$ being nonzero), and $m^*=\text{diag}(Z^{*T}Z^*),$ i.e., 
\end{Proposition}
{\bf Remark: }The proposition implies if the first $r-2$ clusters are more connected within each cluster than the last two clusters and the connection between first $r-2$ clusters and last two clusters are weak, we can find a range for $\lambda$ that leads to merging the last two clusters with high probability. The results can be generalized to merging several clusters at one time. The result above highlights the importance of selecting $\lambda$ as it affects the performance of \ref{SDP:YD} significantly. 

\begin{proof}
	We develop sufficient conditions with a contruction of the dual certificate which guarantees $X^*$ to be the optimal solution. 
	The KKT conditions can be written as below:
	
	First order stationary:
	$$-A -\Lambda +\lambda E_n-\text{diag}(\beta) - \Gamma=0$$
	Primal feasibility:
	$$X\succeq 0,  X\geq 0, X_{ii} = { 1}\quad \forall i=1\cdots,n$$
	Dual feasibility:
	$$\Gamma\geq 0, \Lambda \succeq 0$$
	Complementary slackness
	$$\langle \Lambda, X \rangle =0, \Gamma \circ X=0.$$
	
	
	Consider the following construction:
	denote $T_k=C_k, n_k=m_k,$ for $k< r-1$, $T_{r-1}=C_{r-1}\bigcup C_{r}, n_{r-1}=m_{r-1}+m_{r}$.
	$$X_{T_k}=E_{n_k}$$
	$$X_{T_k T_l}=0,\text{for } k\neq l\leq r-1$$
	
	
	$$\Lambda _{T_k}=-A_{T_k}+\lambda E_{n_k} - \lambda n_k I_{n_k} + \text{diag}(A_{T_k}{\bf 1}_{n_k})$$
	
	$$\Lambda_{T_k T_l}=-A_{T_k, T_l} + \frac{1}{n_l}A_{T_k, T_l}E_{n_l} + \frac{1}{n_k} E_{n_k}A_{T_k,T_l} - \frac{1}{n_ln_k}E_{n_k}A_{T_k, T_l}E_{n_l}$$
	$$\Gamma_{T_k}=0$$
	$$\Gamma_{T_k, T_l}=\lambda E_{n_k, n_l}- \frac{1}{n_l}A_{T_k, T_l}E_{n_l} - \frac{1}{n_k}E_{n_k}A_{T_k,T_l}+\frac{1}{n_ln_k}E_{n_k}A_{T_k, T_l}E_{n_l}$$
	$$\beta = \text{diag}(-A -\Lambda +\lambda E_n - \Gamma)$$
	
	All the KKT conditions are satisfied by construction except for positive semidefiniteness of $\Lambda$ and positiveness of $\Gamma$. Now, we show it one by one.
	
	{\bf Positive Semidefiniteness of $\Lambda$}  \space \space Since $\text{span}(1_{T_k})\subset \text{ker}(\Lambda)$, it suffices to show that for any $u\in span(1_{T_k})^\perp, u^T\Lambda u\geq 0$. Consider $u=\sum_k u_{T_k},$ where $u_{T_k}:=u\circ 1_{T_k}$, then $u_{T_k}\perp 1_{n_k}$.
	\begin{equation}
	\begin{split}
	u^T\Lambda u=&-\sum_k u_{T_k}^TA_{T_k}u_{T_k} - \lambda \sum_k n_k u_{T_k}^T u_{T_k}  + \sum_k u_{T_k}^T \text{diag}(A_{T_k}{\bf 1}_{n_k})u_{T_k}  - \sum_{k\neq l}u_{T_k}^TA_{T_k T_l}u_{T_l}\\
	& =-u^T (A-P)u^T - u^T P u - \lambda \sum_k n_k u_{T_k}^T u_{T_k}  + \sum_k u_{T_k}^T \text{diag}(A_{T_k}{\bf 1}_{n_k})u_{T_k}  \\
	&=-u^T(A-P)u -u_{T_{k-1}}^TP_{T_{k-1}T_{k-1}}u_{T_{k-1}}  - \lambda \sum_k n_k u_{T_k}^T u_{T_k}  + \sum_k u_{T_k}^T \text{diag}(A_{T_k}{\bf 1}_{n_k})u_{T_k} \\
	\end{split}\label{eq:pslambda1}
	\end{equation}
	For the first term, we know
	$$u^T(A-P)u \leq \norm{A-P}_2 \norm{u}_2^2\leq O(\sqrt{n\rho})\norm{u}_2^2 $$ with high probability.
	
	For the second term, and note that $T_{r-1}=C_{r-1}\bigcup C_{r}$, and $$P_{T_{r-1}T_{r-1}} = \begin{bmatrix}
	B_{r-1,r-1}E_{m_{r-1}m_{r-1}}, B_{r-1,r}E_{m_{r-1}m_{r}}\\
	B_{r,r-1}E_{m_rm_{r-1}}, B_{r,r}E_{m_{r}m_{r}}
	\end{bmatrix}$$
	Since $u_{T_{r-1}}\perp 1_{n_{r-1}}$, $$u_{T_{r-1}}^T \begin{bmatrix}
	B_{r-1,r}E_{m_{r-1}m_{r-1}}, B_{r-1,r}E_{m_{r-1}m_{r}}\\
	B_{r,r-1}E_{m_rm_{r-1}}, B_{r,r-1}E_{m_{r}m_{r}}
	\end{bmatrix} u_{T_{r-1}}=0,$$
	therefore 
	\begin{equation}
	\begin{split}
	u_{T_{r-1}}^TP_{T_{r-1}T_{r-1}}u_{T_{r-1}}&=u_{T_{r-1}}^T \begin{bmatrix}
	(B_{r-1,r}-B_{r-1,r-1})E_{m_{r-1}m_{r-1}},0\\
	0, (B_{r-1,r}-B_{r,r})E_{m_rm_{r}}
	\end{bmatrix}u_{T_{r-1}}\\
	&\leq \max \{m_{r-1}(B_{r-1,r-1}-B_{r-1,r}), m_{r}(B_{r,r}-B_{r,r-1})\}\norm{u}_2^2
	\end{split}
	\end{equation}
	
	Consider the last term $ \sum_k u_{T_k}^T \text{diag}(A_{T_k}{\bf 1}_{n_k})u_{T_k} $. Using Chernoff, we know
	$$||\text{diag}(A_{T_k} {\bf 1}_{n_k})||_2 \geq B_{k,k}^* n_k - \sqrt{6\rho n_k\log n_k}$$ with high probability,
	where for $k, l<r-1$, $$B_{kl}^*=B_{kl},$$ 
	$$B_{k,r-1}^*=\frac{m_{r-1}B_{k,r-1}+m_r B_{k,r}}{m_{r-1}+m_r},$$
	$$B_{r-1,r-1}^*=\frac{(m_{r-1}^2B_{r-1,r-1}+2*m_r m_{r-1}B_{r-1,r}+(m_{r}^2B_{r,r})}{(m_{r-1}+m_r)^2}.$$
	%Therefore, a sufficient condition is:
% 	\begin{equation}\label{eq:lb1}
% 	\lambda\geq \Omega(\sqrt{np_{max}})+\max \{m_{r-1}(B_{r-1,r-1}-B_{r-1,r}), m_{r}(B_{r,r}-B_{r,r-1})\}
% 	\end{equation}
	
	Therefore, :
	$$- \lambda \sum_k n_k u_{T_k}^T u_{T_k}  + \sum_k u_{T_k}^T \text{diag}(A_{T_k}{\bf 1}_{n_k})u_{T_k}\geq \min_k({B_{k,k}^*n_k-\Omega(\sqrt{\rho n_k\log n}) - \lambda n_k}) \norm{u}_2^2.$$
	
	So with equation~\ref{eq:pslambda1}, a sufficient condition for positive semidefiniteness of $\Lambda$ is $$\min_k({B_{k,k}^*n_k-\Omega(\sqrt{\rho n_k\log n}) - \lambda n_k}) \geq O(\sqrt{n\rho}) +\max  \{m_{r-1}(B_{r-1,r-1}-B_{r-1,r}), m_{r}(B_{r,r}-B_{r,r-1})\}$$
	
	which implies,  $$\lambda \leq \min_k B_{kk}^* -\max_k \max \{\frac{m_{r-1}}{n_k}(B_{r-1,r-1}-B_{r-1,r}), \frac{m_{r}}{n_k}(B_{r,r}-B_{r,r-1})\}+ O( \sqrt{\rho n \log n})$$
	
	
	{\bf Positiveness of $\Gamma$}  $$\mathbb{E}[\Gamma_{T_k, T_l}]=(\lambda - B^*_{k,l})E_{n_k, n_l}.$$
	
	
	
	Using Chernoff bound, we know $\Gamma_{T_k, T_l} > 0$ with high probability as long as $\lambda \geq \max_{k\neq l}B^*_{k,l} + \Omega(\sqrt{\rho \log n /n\pi_\text{min}})$. 
	
	
	
\end{proof}

%\section{Proofs for \ref{SDP:BW}}
\section{Additional Theoretical Results and Proofs of Results in Section~\ref{sec:uknownk}}
\label{sec:proofformatrcv}

\subsection{Proof of Theorem~\ref{thm:matrcv_general}}

\begin{proof}
With probability greater than $1-\delta_\text{est}-\delta_\text{over}-\delta_\text{under}$, the following three inequalities hold.

For $r_T\geq r_t > r:$
\begin{align*}
    \langle \hat{S}^{22}, \hat{X}^{22}_{r} \rangle& \geq  \langle \hat{S}^{22}, X_0^{22} \rangle -\epsilon_\text{est} \geq \max_{r_T\geq r_t >r} \langle \hat{S}^{22}, \hat{X}^{22}_{r_t}\rangle  -\epsilon_\text{est} - \epsilon_\text{over}\\
    & \geq \max_{r_T\geq r_t >r}\langle \hat{S}^{22}, \hat{X}^{22}_{r_t}\rangle - \Delta  \\
    %& \geq \max_{\hat{r}\in R, \hat{r} >r}\langle \hat{S}^{22}, \hat{X}^{22}_{\hat{r}}\rangle - \Delta.
\end{align*}

For $r_t < r:$
\begin{align*}
    \langle \hat{S}^{22}, \hat{X}^{22}_{r} \rangle& \geq \langle \hat{S}^{22}, X_0^{22} \rangle -\epsilon_\text{est} \geq \max_{ r_t <r}\langle \hat{S}^{22}, \hat{X}^{22}_{r_t}\rangle  -\epsilon_\text{est} + \epsilon_\text{under}\\
    & > \max_{ r_t <r}\langle \hat{S}^{22}, \hat{X}^{22}_{r_t}\rangle + \Delta  \\
    %& \geq \max_{\hat{r}\in R, \hat{r}<r} \langle \hat{S}^{22}, \hat{X}^{22}_{ \hat{r}}\rangle - \Delta.
\end{align*}



Therefore, with probability at least $1-\delta_\text{est}-\delta_\text{over}-\delta_\text{under}$, $\langle \hat{S}^{22}, \hat{X}^{22}_{r} \rangle \geq \max_{t} \langle \hat{S}^{22}, \hat{X}^{22}_{r_t} \rangle -\Delta$. Let  $R= \{r_t: \langle \hat{S}^{22}, \hat{X}^{22}_{r_t} \rangle \geq \max_t \langle \hat{S}^{22}, \hat{X}^{22}_{r_t} \rangle - \Delta\}$. It follows then $r\in R$.

Furthermore, with probabiltiy at least $1-\delta_\text{est}-\delta_\text{under}$, for $r_t < r:$
\begin{align*}
    \langle \hat{S}^{22}, \hat{X}^{22}_{r_t} \rangle& \leq  \langle \hat{S}^{22}, X_0^{22}\rangle - \epsilon_\text{under} \leq \langle \hat{S}^{22}, \hat{X}^{22}_{r}\rangle  +\epsilon_\text{est} - \epsilon_\text{under}\\
    & < \max_t \langle \hat{S}^{22}, \hat{X}^{22}_{r_t} \rangle - \Delta.
\end{align*}
Therefore, for any $r_t< r$, $r_t\notin R$, and $\min\{r_t: r_t\in R\}=r$.
\end{proof}



\subsection{Range of $\lambda$ for merging clusters in \ref{SDP:BW-lambda}}
\label{sec:merge2}
\cite{yan2017provable} proved consistency result of \ref{SDP:BW} for a range of $\lambda$. 
%The paper shows, if $c_1\max_{k} \sqrt{m_k B_{kk}} + c_2 \sqrt{n \max_{k\neq \ell} B_{k\ell}} \leq\lambda \leq m_\text{min} (\delta -\max _{k,\ell} \sqrt{\frac{B_{k\ell}\log m_k}{m_k}}),$
%then $\tilde{X}$ 
%equals the true normalized clustering matrix with high probability, if $\delta \geq 2\sqrt{6\log n} \max_k \sqrt{\frac{B_{kk}}{m_k}} + 6 \max_{\ell\neq k} \sqrt{\frac{B_{k\ell}\log n}{m_{\text{min}}}} + \frac{c\sqrt{n p_\text{max}}}{m_\text{min}}$, $\delta =\min_{k} (B_{kk}-\max_{\ell\neq k} B_{k\ell})$.
Here, we show that for $\lambda$ in a different range, the SDP will return a merged clustering matrix with high probability. %i.e., $\text{trace}(\tilde{X})<r$.
Specifically, we present the conditions for $\lambda$ that return $\text{trace}(\tilde{X})=r-1$, meaning that the \ref{SDP:BW} would merge two clusters into one. The results can be generalized to merging several clusters at one time as well. %For example, how hierarchical model, we can get the conditions for $\lambda$ such that \ref{SDP:BW} would merge all sub-clusters into one at the same time. 

\begin{Proposition}\label{prop:sdp2merge}
	Let $\tilde{X}$ be the optimal solution of \ref{SDP:BW} for $A\sim SBM(B,Z)$. Suppose
	$\lambda \leq  O(\pi_\text{min}^2n \min_{k\neq l}(B_{kk}-B_{kl}))- \Omega(\sqrt{\rho n \log n/\pi_\text{min}})$, and for every $k<r-1, $
	\begin{equation}
	\begin{split}
	&\Omega(\sqrt{n\rho})+\max \{m_{r-1}(B_{r-1,r-1}-B_{r-1,r}), m_{r}(B_{r,r}-B_{r,r-1})\}\leq\lambda \\
	&\leq  \frac{(m_km_{r-1} + m_km_r)(B_{k,k}+B_{r-1,r-1}^*-2B_{k,r-1}^*)}{m_k + m_{r-1} + m_r}- \Omega(\sqrt{\rho \pi_\text{min}n \log n}),
	\end{split}
	\end{equation}
	then $\tilde{X}=X^*$ with high probability, where $X^*$ is the normalized clustering matrix when the last two clusters are merged, and $B^*$ is the $(r-1)\times( r-1)$ corresponding clustering probability matrix. %is the $(r-1)\times( r-1)$ clustering probability matrix after the last two clusters are merged, i.e., for
$k, l<r-1$, $B_{kl}^*=B_{kl},$ $B_{k,r-1}^*=\frac{m_{r-1}B_{k,r-1}+m_K B_{k,r}}{m_{r-1}+m_r},$ $B_{r-1,r-1}^*=\frac{(m_{r-1}^2B_{r-1,K-1}+2*m_r m_{r-1}B_{r-1,r}+(m_{r}^2B_{r,r})}{(m_{r-1}+m_r)^2}.$
	% $X^*=Z^*\text{diag}(m^*)^{-1}Z^{*T}$, $Z^*=Z(I-E_{K,K}+E_{K,K-1})$($E_{i,j}$ is the matrix only with $E_{ij}=1$ being nonzero), and $m^*=\text{diag}(Z^{*T}Z^*),$ i.e., 
\end{Proposition}
{\bf Remark: }The proposition implies appropriate conditions on the connectivity patterns of the graph can lead to merged clusters if $\lambda$ is not chosen correctly, similar in spirit to Proposition \ref{prop:sdp1merge}.


\begin{cor}\label{cor:sdp2merge1}
Uneven separations: for a SBM with $m_1 = \cdots =m_r$, and $B_{1,1}=p_1 \geq B_{2,2}=p_2 \geq \cdots B_{r,r}=p_r $, and $B_{k,l}=q$ for $k\neq l$. The condition for $\lambda$ to merge the last two clusters is $$\Omega(\sqrt{n\rho})+m(p_{r-1}-q)\leq\lambda 
\leq  (4p_{r-2}+p_{r-1}+p_{r}-6q)m/6- \Omega(\sqrt{\rho n \log n}),$$
the interval is nonempty when $n$ is large, $p,q=\Theta(1), m_k=\Theta(n)$ and $p_{r-2}\geq \frac{5p_{r-1}-p_{r}}{4};$
\end{cor}
\begin{cor}\label{cor:sdp2merge2}
Uneven cluster sizes: for a SBM with $m_1 = \cdots =m_{r-2}=m\geq m_{r-1}=m_r = m^*$ and $B_{k,k}=p $, and $B_{k,l}=q$ for $k\neq l$. The condition for $\lambda$ to merge the last two clusters is $$\Omega(\sqrt{n\rho})+m^*(p-q)\leq\lambda 
\leq  \frac{3mm^*(p-q)}{4m^*+2m}- \Omega(\rho n \log n),$$
the interval is nonempty when $n$ is large, $p,q=\Theta(1), m, m^*=\Theta(n)$ and $\frac{m^*}{m}\leq \frac{3-\sqrt{2}}{2\sqrt{2}}.$
\end{cor}
%\subsection{Proofs of Proposition \ref{prop:sdp2merge}, Corollary \ref{cor:sdp2merge1} and Corollary \ref{cor:sdp2merge2}}
%\label{sec:merge2}
\begin{proof}[Proof of Proposition \ref{prop:sdp2merge}]
We develop sufficient conditions with a construction of the dual certificate which guarantees $X^*$ to be the optimal solution. 
The KKT conditions can be written as below:

First order stationary:
$$-A -\Lambda +(1\alpha^T+\alpha 1^T)+\beta I - \Gamma$$
Primal feasibility:
$$X\succeq 0, X\geq 0, X{\bf 1}_n={\bf 1}_n, \text{trace}(X) = r$$
Dual feasibility:
$$\Gamma\geq 0, \Lambda \succeq 0$$
Complementary slackness
$$\langle \Lambda, X \rangle =0, \Gamma \circ X=0.$$


Consider the following construction:
denote $T_k=C_k, n_k=m_k,$ for $k< r-1$, $T_{r-1}=C_{r-1}\bigcup C_{r}, n_{r-1}=m_{r-1}+m_{r}$.
$$X_{T_k}=E_{n_k}/n_k$$
$$X_{T_k T_l}=0,\text{for } k\neq l\leq r-1$$
$$\Lambda _{T_k}=-A_{T_k}+(1_{n_k}\alpha_{T_k}^T+\alpha_{T_k}1_{n_k}^T)+\lambda I_{n_k}$$
$$\Lambda_{T_k T_l}=-(I-\frac{E_{n_k}}{n_k})A_{T_k T_l}(I-\frac{E_{n_l}}{n_l})$$
$$\Gamma_{T_k}=0$$
$$\Gamma_{T_k, T_l}=-A_{T_kT_l}-\Lambda_{T_kT_l}+(1_{n_k}\alpha_{T_l}^T+\alpha_{T_k}1_{n_l}^T)$$
$$\alpha_{T_k}=\frac{1}{n_k}(A_{T_k}1_{n_k}+\phi_k1_{n_k})$$
$$\phi_k=-\frac 12 (\beta+\frac{1_{n_k}^TA_{T_k}1_{n_k}}{n_k})$$

All the KKT conditions are satisfied by construction except for positive semidefiniteness of $\Lambda$ and positiveness of $\Gamma$. Now, we show it one by one.

{\bf Positive Semidefiniteness of $\Lambda$}  \space \space Since $\text{span}(1_{T_k})\subset \text{ker}(\Lambda)$, it suffices to show that for any $u\in span(1_{T_k})^\perp, u^T\Lambda u\geq 0$. Consider $u=\sum_k u_{T_k},$ where $u_{T_k}:=u\circ 1_{T_k}$, then $u_{T_k}\perp 1_{n_k}$.
\begin{equation}
\begin{split}
    u^T\Lambda u=&-\sum_k u_{T_k}^TA_{T_k}u_{T_k} + \lambda \sum_k u_{T_k}^T u_{T_k} - \sum_{k\neq l}u_{T_k}^TA_{T_k T_l}u_{T_l}\\
    & =-\sum_k u_{T_k}^T(A-P)_{T_k}u_{T_k} - \sum_{k\neq l}u_{T_k}^T(A-P)_{T_k T_l}u_{T_l}+ \lambda \norm{u}_2^2 - u^TPu\\
    &=-u^T(A-P)u + \lambda \norm{u}_2^2 - u_{T_{r-1}}^TP_{T_{r-1}T_{r-1}}u_{T_{r-1}}\\
\end{split}
\end{equation}
Now consider $u_{T_{r-1}}^TP_{T_{r-1}T_{r-1}}u_{T_{r-1}}$, and note that $T_{r-1}=C_{r-1}\bigcup C_{r}$, and $$P_{T_{r-1}T_{r-1}} = \begin{bmatrix}
B_{r-1,r-1}E_{m_{r-1}m_{r-1}}, B_{r-1,r}E_{m_{r-1}m_{r}}\\
B_{r,r-1}E_{m_rm_{r-1}}, B_{r,r}E_{m_{r}m_{r}}
\end{bmatrix}$$
Since $u_{T_{r-1}}\perp 1_{n_{r-1}}$, $$u_{T_{r-1}}^T \begin{bmatrix}
B_{r-1,r}E_{m_{r-1}m_{r-1}}, B_{r-1,r}E_{m_{r-1}m_{r}}\\
B_{r,r-1}E_{m_rm_{r-1}}, B_{r,r-1}E_{m_{r}m_{r}}
\end{bmatrix} u_{T_{r-1}}=0,$$
therefore 
\begin{equation}
\begin{split}
    u_{T_{r-1}}^TP_{T_{r-1}T_{r-1}}u_{T_{r-1}}&=u_{T_{r-1}}^T \begin{bmatrix}
(B_{r-1,r}-B_{r-1,r-1})E_{m_{r-1}m_{r-1}},0\\
0, (B_{r-1,r}-B_{r,r})E_{m_rm_{r}}
\end{bmatrix}u_{T_{r-1}}\\
&\leq \max \{m_{r-1}(B_{r-1,r-1}-B_{r-1,r}), m_{r}(B_{r,r}-B_{r,r-1})\}\norm{u}_2^2
\end{split}
\end{equation}
Since $\norm{A-P}\leq c_0\sqrt{np}$ provided $p\geq c_0 \log n/n$,
Therefore, a sufficient condition is:
\begin{equation}\label{eq:lb2}
    \lambda\geq \Omega(\sqrt{np_{max}})+\max \{m_{r-1}(B_{r-1,r-1}-B_{r-1,r}), m_{r}(B_{r,r}-B_{r,r-1})\}
\end{equation}


{\bf Positiveness of $\Gamma$}  \space \space Define $d_i^*(T_k)=\sum_{j\in T_k}A_{i,j}$, $\bar{d}_i^*(T_k)=\frac{d_{i}^*(T_k)}{n_k}$, and $\bar{d}^*(T_k T_l)=\frac{\sum_{i\in T_l}\bar{d}_i^*(T_k)}{n_l}.$ 
Then consider $x\in T_{k}$, $y\in T_{l}$, we need
$$\bar{d}_x^*(T_k)-\bar{d}_x^*(T_l)+\frac 12 (\bar{d}^*(T_kT_l)-\bar{d}^*(T_kT_k))+\bar{d}_y^*(T_l)-\bar{d}_y^*(T_k)+\frac 12 (\bar{d}^*(T_kT_l)-\bar{d}^*(T_lT_l))-\frac{\lambda}{2n_l} - \frac{\lambda}{2n_k}\geq 0,$$

Using Chernoff bound, for positiveness of $\Gamma$ with high probability we only need $$\frac{1}{2}(B_{kk}^*+B_{ll}^*-2B_{kl}^*)-\sqrt{6\log n }(\sqrt{\frac{B_{kk}^*}{n_k}}+\sqrt{\frac{B_{ll}^*}{n_l}})-\sqrt{18B_{kl}^*\log n (\frac{1}{n_k}+\frac{1}{n_l})}\geq \frac{\lambda}{2n_l}+\frac{\lambda}{2n_k}$$

where for $k, l<r-1$, $$B_{kl}^*=B_{kl},$$ 
$$B_{k,r-1}^*=\frac{m_{r-1}B_{k,r-1}+m_r B_{k,r}}{m_{r-1}+m_r},$$
$$B_{r-1,r-1}^*=\frac{(m_{r-1}^2B_{r-1,r-1}+2*m_r m_{r-1}B_{r-1,r}+(m_{r}^2B_{r,r})}{(m_{r-1}+m_r)^2}.$$
If ${k,l}< {r-1}$, then $B_{kl}^*=B_{kl}, n_l=m_l$, the condition becomes
$$\frac{1}{2}(B_{kk}+B_{ll}-2B_{kl})-\sqrt{6\log n }(\sqrt{\frac{B_{kk}}{m_k}}+\sqrt{\frac{B_{ll}}{m_l}})-\sqrt{18B_{kl}\log n (\frac{1}{m_k}+\frac{1}{m_l})}\geq \frac{\lambda}{2m_l}+\frac{\lambda}{2m_k},$$

which is equivalent to $$\lambda \leq  O(\pi_\text{min}^2n \min_{k\neq l}(B_{kk}-B_{kl}))- \Omega(\sqrt{\rho n \log n/\pi_\text{min}}).$$


Now, suppose $k<r-1, l=r-1$, the condition becomes:
\begin{equation}
\begin{split}
\label{eq:1}
\frac{1}{2}(B_{kk}+B_{ll}^*-2B_{kl}^*)&-\sqrt{6\log n }(\sqrt{\frac{B_{kk}}{m_k}}+\sqrt{\frac{B_{ll}^*}{m_{r-1}+m_r}})\\
&-\sqrt{18B_{kl}^*\log n (\frac{1}{m_k}+\frac{1}{m_{r-1}+m_{r}})}\geq \frac{\lambda}{2m_{r-1}+2m_{r}}+\frac{\lambda}{2m_k}.
\end{split}
\end{equation}

Since $\sqrt{6\log n }(\sqrt{\frac{B_{kk}}{m_k}}+\sqrt{\frac{B_{ll}^*}{m_{r-1}+m_r}})\frac{m_k(m_{r-1} + m_r)}{m_k+ m_{r-1} + m_r} = O(\sqrt{\rho n \log n/\pi_\text{min} }),$ and similarly for other terms, then we have the sufficient condition for positiveness of $\Gamma$ on $\lambda$:
$$\lambda \leq  \frac{(m_km_{r-1} + m_km_r)(B_{k,k}+B_{r-1,r-1}^*-2B_{k,r-1}^*)}{m_k + m_{r-1} + m_r}- \Omega(\sqrt{\rho n \log n/\pi_\text{min}}).$$
\end{proof}


%Corrollary:
\begin{proof}[Proof of Corollary~\ref{cor:sdp2merge1}]
%{\bf Equal-sized with different $p$ case: } 
Now suppose we have equal sized clusters, with $p_1\geq p_2\geq p_3\geq...\geq p_r$ for within cluster probability. Assume $q$ for between cluster probability. Consider fixed $r$, $m_r=n/r=m$, and assume dense graph: $p_i,q=\Theta(1)$,
then we can drop the negative term in equation \ref{eq:1}, we have:
$$\lambda \geq \norm{A-P} + m (p_{r-1}-q)$$
$$\frac 12 (p_{r-2} + \frac{p_{r-1}+p_{r}+2q}{4}-2q)\geq \frac{3\lambda}{4m},$$
if we drop $\norm{A-P}$, we get $$P_{r-2}\geq \frac{5P_{r-1}-P_{r}}{4},$$
if $P_{r-1}=P_K$, then it becomes $$P_{r-2}\geq P_{r-1}$$
Actually, for this simple case, we can show that to merge the last $r$ clusters, the bound would be: 
$$\lambda \geq \norm{A-P} + m(p_{r-r +1}-q)$$
$$\frac{1}{2}(p_{r-r} + \frac{\sum_{i=r-r+1}^Kp_i+(r^2-r)q} {r^2}-2q)\geq \frac{\lambda (r+1)}{2mr}.$$

We can show that $$m(p_{r-r}-q)\geq \frac{1}{2}(p_{r-r} + \frac{\sum_{i=r-r+1}^Kp_i+(r^2-r)q} {r^2}-2q),$$
i.e. the upper bound for merging the last $r$ clusters is less than the lower bound for merging the last $r+1$ clusters. 
\end{proof}


 %{\bf Unbalanced-sized case: } 
 \begin{proof}[Proof of Corollary~\ref{cor:sdp2merge2}]
 Now let's assume $p'=p, q'=q$, while relaxing the equal size constrain: assume the last two cluster of size $m^*$. Then above requirement becomes:
 $$\frac 34 (p-q)\geq \frac{\sqrt{2}}{4}(p-q) + \frac{\sqrt{2}m^*(p-q)}{2m},$$
 i.e. $\frac{m^*}{m}\leq \frac{3-\sqrt{2}}{2\sqrt{2}}.$
 %In conclusion, the range for $\lambda$ is not empty if the $SBM$ has not well-separated clusters or has small clusters. In either case, SDP will merge those clusters with high probability given the $\lambda$ within the range.

\end{proof}

\begin{remark}
The analysis can be easily generalized to hierarchical model showing the range such that several clusters are merged at the same time. Consider the model described in~\cite{Li2018hierarchical} (Definition 1), and assume equal size $m$, and a dense degree regime. Then we can still apply the primal-dual certificate proof with another construction. In this case of binary tree SBM, intuitively, we would merge those clusters such that $s(x,x')=1$ first. Suppose the depth of the tree is $d$. Then define $T_1 = S_{0,0,0,...,0}\bigcup S_{1,0,0,...,0}$, $T_2 = S_{0,1,0,...,0}\bigcup S_{1,1,0,...,0}$,...,$T_{2^{d-1}}=S_{0,1,...,1}\bigcup S_{1,1...,1}$, where $S_{id}$ is a cluster indexed by a binary index $id$. Using a similar proof, we can get a range for $\lambda$ such that $X$ corresponds to $T$ is the optimal solution for the SDP. 

The only changes in the proof would be as follows:

(1) for the lower bound of $\lambda$, $u^TPu$ is not zero.

\begin{equation}
    \begin{split}
        u^TPu &= \sum_{j,k}u_j^T P_{j,k}u_k = \sum_k u_k^T P_{k,k}u_k + \sum_{j\neq k}u_j^T P_{j,k}u_k \\
        &= \sum_k u_k^T\begin{bmatrix}
p_0 E_m, p_1E_m\\
p_1 E_m, p_0 E_m
\end{bmatrix}u_k + \sum_{j\neq k}u_j^T P_{j,k}u_k\\
    \end{split}
\end{equation}
Due to the binary tree structure, $P_{j,k}$ is a constant matrix, so off-diagonal terms will go away, and following similar arguments the diagonal term is bounded by $(p_0-p_1)m$. 

Therefore the lower bound for $\lambda$ is:
$$\lambda\geq \sqrt{np_{max}} + (p_0-p_1)m.$$

%Basically, we need $B^*_{ll}>B^*_{kl}$, $B_{kk}>B^*_{kl}$, which means $k'th$ cluster should be well separated from the last two clusters. 
(2) the upper bound of $\lambda$ becomes (drop the negative terms):

$$\frac 12 (\frac{p_0+p_1}{2} + \frac{p_0+p_1}{2}-p_2)\geq \frac{\lambda}{2m}.$$

Combining them together, we have:

$$(p_0+p_1-2p_2)m \geq \lambda \geq (p_0-p_1)m$$
\end{remark} 
%\subsection{Proofs of theoretical results in Section~\ref{sec:matrcv_sbm}}
%\label{sec:prop4thm5}

\subsection{Proof of Theorem~\ref{cor:nok}}

We first prove a concentration lemma that holds for any normalized clustering matrix $X$ independent of $A$.
% \begin{lemma}\label{lem:abound}
% Consider a $A$ generated from a $SBM(Z,B)$ with $r$ clusters. Let $X\in \mathcal{C}_{k_0}$ be a normalized clustering matrix independent of $A$. \rd Then $\langle A, X\rangle\leq \sqrt{k_0\rho\log n}$ with probability tending to one. \bk
% \end{lemma}
% \begin{proof}
% Let $S_k$ denote the clusters induced by $X$.
% Note that due to the independence between $A$ and $X$, 
% \begin{align*}
% \var(\langle A-P,X \rangle) &= \var (\sum_k \sum_{i,j\in S_k} (A_{ij}-P_{ij})/|S_k| )\\
% &=4\var(\sum_k \sum_{i,j\in S_k, i<j} (A_{ij}-P_{ij})/|S_k| )\\
% &\leq \sum_k \sum_{i,j\in S_k, i<j} \frac{\rho}{|S_k|^2}
% =O (k_0 \rho)
% \end{align*}
% \end{proof}

\begin{lemma}\label{lem:generalsamplebound}
Consider a an adjacency matrix $A$ and its population version $P$. Let $X$ be a normalized clustering matrix independent of $A$. Then with  probability at least $1-O(n^{-1})$, $$| \langle A-P, X \rangle | \leq (1+B_{\max})\sqrt{\tr{X} \log n}$$
%similarly, with high probability ($1-n^{-1}$),
%$$\langle S-\hat{S}, X \rangle \geq -(b-a)\sqrt{\text{trace}(X) \log n/2}.$$% \rd Then $\langle A, X\rangle\leq \sqrt{k_0\rho\log n}$ with probability tending to one. \bk
with $B_{\max}=\max_{i,j}B_{ij}$.
\end{lemma}
\begin{proof}
The result follows from Hoeffding's inequality and the fact that $X$ is a projection matrix.

By independence between $A$ and $X$, 
\begin{align*}
    P\left(\sum_{i<j} (A_{ij}-P_{ij})X_{ij} > t\right) & \leq \exp (-\frac{2t^2}{(1+B_{\max})^2 \sum_{i< j} X_{ij}^2})\\
    &\leq \exp (-\frac{4t^2}{ (1+B_{\max})^2\norm{X}_F^2})\\
    &=\exp (-\frac{4t^2}{ (1+B_{\max})^2\tr{X}})
\end{align*}
Let $t = \frac{1}{2}(1+B_{\max})\sqrt{\text{trace}(X) \log{n}}$, then by symmetry in $A$ and $X$, $P(\langle A-P, X \rangle > (1+B_{\max})\sqrt{\text{trace}(X) \log{n}} ) = O(1/n).$ The other direction is the same.




%and similarly $\var(\langle A^{22} -P^{22}, X^{22} \rangle) = \mathcal{O} (\hat{r} \rho)$.

%Then with Chebyshev, $\langle A -P, X \rangle\geq -C \sqrt{r \rho \log n}$ and $\langle A^{22} -P^{22}, X^{22} \rangle\leq C \sqrt{\rho\hat{r}\log n} \leq C \sqrt{\rho\sqrt{n}\log n}$ with high probability. 
\end{proof}

% \begin{lemma}
% \label{lem:lambda-monotone}
%     For \ref{SDP:BW}, if $\lambda_1>\lambda_2$, we have 
%     $$\text{trace}(\tilde{X}_2)\geq \text{trace}(\tilde{X}_1),$$
%     where $\tilde{X}_1$ and $\tilde{X}_2$ are the normalized clustering matrix returned from \ref{SDP:BW} corresponding to $\lambda_1$ and $\lambda_2$.
% \end{lemma}
% \begin{proof}
%     Because $\tilde{X}_1$ and $\tilde{X}_2$ are optimal solutions for \ref{SDP:BW} with $\lambda_1$ and $\lambda_2$ respectively, we have
%     \begin{equation}
%         \langle A,\tilde{X}_1\rangle -\lambda_1\text{trace}(\tilde{X}_1)\geq  \langle A,\tilde{X}_2\rangle -\lambda_1\text{trace}(\tilde{X}_2),
%     \end{equation}
%     and similarly we have
%     \begin{equation}
%         \langle A,\tilde{X}_2\rangle -\lambda_2\text{trace}(\tilde{X}_2)\geq  \langle A,\tilde{X}_1\rangle -\lambda_2\text{trace}(\tilde{X}_1).
%     \end{equation}
%     Combine them together, we have
%     \begin{equation}
%         \lambda_2\text{trace}(\tilde{X}_2-\tilde{X}_1)\leq \langle A,\tilde{X}_2-\tilde{X}_1\rangle \leq \lambda_1\text{trace}(\tilde{X}_2-\tilde{X}_1),
%     \end{equation}
%     which implies that $\text{trace}(\tilde{X}_2)\geq \text{trace}(\tilde{X}_1)$.
% \end{proof}

%Before proving proposition~\ref{prop:underestimate}, proposition~\ref{prop:overestimate} and proposition~\ref{prop:sdp_exactrecovery}, we present a lemma which will help the proofs.


In order to prove Theorem~\ref{cor:nok}, we need to derive the three error bounds in Theorem~\ref{thm:matrcv_general} in this setting. For notational convenience, we first derive the bounds for $A$ and a general normalized clustering matrix $\hat{X}$, with the understanding that the same asymptotic bounds apply to estimates obtained from the training graph provided the split is random and the number of training nodes is $\Theta(n)$.

\begin{lemma}\label{prop:underestimate}
For a sequence of underfitting normalized clustering matrix $\{\hat{X}_{r_t}\}_{r_t<r}$, all independent of $A$,  provided $n\rho/\sqrt{log n} \to \infty$, we have
\begin{equation*}
   \max_{r_t <r} \langle A, \hat{X}_{r_t}\rangle \leq \langle A, X_0\rangle- \Omega_P(n\rho \pi_{\text{min}}^2 /r^2),
\end{equation*}
for fixed $r$ and $\pi_{\min}$.
\end{lemma}



\begin{proof}
%Denote $\tilde{S}_{i,j} = \max_{\{k,\ell|k \in C(i),\ell\in C(j)\}} S_{k,\ell}$, where $C(i)$ is the cluster that node $i$ belongs to, as the induced block-wise constant matrix from $S$, and $H_{i,j} = \tilde{S}_{\{k,\ell|\forall k\in C_i,\ell\in C_j\}}$.

Let $\{\hat{C}_k\}$ be the clusters associated with $\hat{X}$. Denote $\gamma_{k,i} = |\hat{C_k} \cap C_i|$, and $\hat{m}_k = |\hat{C}_k| = \sum_i \gamma_{k,i}$, $r_t = \text{rank}(\hat{X})< r.$ First note that for each $i\in [r]$, $\exists k\in [r_t]$, s.t. $\gamma_{k,i}\geq |C_i|/r_t$. Since $r>r_t$, by the Pigeonhole principle, we see that $\exists i_0,j_0,k_0$, $i_0\neq j_0$, such that,     

%First note that by $\exists k, |\hat{C}_k|>n\pi_{\min}$. Now note that using the Pigeonhole principle, if $\hat{C}_k$ has an intersection with $r_0$ of the ground truth clusters, then $\gamma_{k,i}\leq n\pi_{\min}/r_0$. 
%there exists $k_0, i_0, j_0$, such that
$$\gamma_{k_0, i_0}=|\hat{C}_{k_0} \cap C_{i_0}| \geq |C_{i_0}| / r_t \geq \pi_\text{min} n/ r_t$$
\begin{align}
    \gamma_{k_0, j_0}=|\hat{C}_{k_0} \cap C_{j_0}| \geq |C_{j_0}| / r_t \geq \pi_\text{min} n/ r_t
    \label{eq:pigeonhole}
\end{align}




For each $k\neq k_0$, 
$$ \frac{\sum_{i,j} B_{i,j} \gamma_{k,i}\gamma_{k,j}}{\hat{m}_k} \leq \frac{\sum_{i} B_{i,i} \sum_j \gamma_{k,i}\gamma_{k,j}}{\hat{m}_k} = \sum_{i} B_{i,i}\gamma_{k,i}.$$

For $k= k_0$, 

\begin{equation}
\begin{split}
        \frac{\sum_{i,j} B_{i,j} \gamma_{k,i}\gamma_{k,j}}{\hat{m}_k} & = \frac{\sum_{i,j} B_{i,i} \gamma_{k,i}\gamma_{k,j}}{\hat{m}_k}
+ \frac{\sum_{i\neq j} (B_{i,j} - B_{i,i}) \gamma_{k,i}\gamma_{k,j}}{\hat{m}_k}\\
        & = \sum_{i} B_{i,i}\gamma_{k,i} + \frac{\sum_{i\neq j} (B_{i,j} - B_{i,i})
        \gamma_{k,i}\gamma_{k,j}}{\hat{m}_k}\\
        & \leq \sum_{i} B_{i,i}\gamma_{k,i} + \frac{(2B_{i_0,j_0} - B_{i_0,i_0} - B_{j_0,j_0}) \gamma_{k,i_0}\gamma_{k,j_0}}{\hat{m}_k}\\
        & = \sum_{i} B_{i,i}\gamma_{k,i} - \frac{\left((B_{i_0,i_0}-B_{i_0,j_0})+(B_{j_0,j_0}-B_{i_0,j_0})\right) \gamma_{k,i_0}\gamma_{k,j_0}}{\hat{m}_k}\\
        & \stackrel{(a)}{\leq} \sum_{i} B_{i,i}\gamma_{k,i} - \frac{2\tau\gamma_{k,i_0}\gamma_{k,j_0}}{n\pi_{\text{min}}\hat{m}_k}\\
        & \leq \sum_{i} B_{i,i}\gamma_{k,i} - \frac{2\tau {\pi_{\text{min}}n}}{r_t^2\hat{m}_k},
%        & \leq \sum_{i} B_{i,i}\alpha_{k,i} - \frac{2\tau {\pi_{\text{min}}^2n^2}}{r^2\hat{m}_k},\\
    \end{split}
\end{equation}
where $\tau= n\pi_{\text{min}}p_{\text{gap}}$, $p_{\text{gap}}:=\min_i ( B_{i,i} - \max_{j\neq i} B_{i,j})$.
$(a)$ is true by definition of $\tau$ and Eq~\eqref{eq:pigeonhole}. %because $B_{i_0,i_0}-B_{i_0,j_0}\geq B_{i_0,i_0}-\max_{j\neq i_0}B_{i_0,j}$ and $(B_{i_0,i_0}-B_{i_0,j_0})+(B_{i_0,i_0}-B_{i_0,j_0})\geq \min_i B_{i,i}-\max_{j\neq i}B_{i,j}=:\tau/(n\pi_{\text{min}})$.

Therefore, since $\hat{m}_{k_0}\leq n$,
\begin{align}
    \langle P, \hat{X}\rangle &=  \sum_{k=1}^{r_t} \frac{\sum_{i,j} B_{i,j} \gamma_{k,i}\gamma_{k,j}}{\hat{m}_k} -O(\rho r_t)\leq \sum_{k=1}^{r_t}\sum_{i=1}^r B_{i,i}\gamma_{k,i} - \Omega(\frac{\tau {\pi_{\text{min}} n}} {r_t^2\hat{m}_{k_0}})\notag\\
    &= \langle P, X_0\rangle  - \Omega\left(\frac{\tau {\pi_{\text{min}} }} {r_t^2}\right).
    \label{eq:under_pop_sbm}
\end{align}

Next by Lemma~\ref{lem:generalsamplebound}, for each $X$ with $\tr{X}\leq r$,
\begin{align*}
|\langle A-P, X \rangle| \leq (1+B_{\max})\sqrt{r\log n}    
\end{align*}
with probabiltiy at least $1-O(1/n)$. By a union bound and using the same argument, w.h.p.
\begin{align}
\max_{r_t<r}|\langle A-P, \hat{X}_{r_t} \rangle| \leq (1+B_{\max})\sqrt{r\log n}   \label{eq:union_noise}
\end{align}

Eqs~\eqref{eq:under_pop_sbm} and~\eqref{eq:union_noise} imply w.h.p.
\begin{align}
    & \langle A, X_0\rangle - \max _{r_t<r} \langle A, \hat{X}_{r_t}\rangle    \notag\\ 
    %\geq & \langle P, X_0-\hat{X}\rangle - \max _{\hat{r}<r} |\langle A-P, \hat{X} - X_0\rangle |
    %\nonumber\\
    = & \Omega\left(\frac{np_{gap} {\pi_{\text{min}}^2 }} {r^2}\right) -  O(\sqrt{r\log n}) = \Omega\left(\frac{np_{gap} {\pi_{\text{min}}^2 }} {r^2}\right) \label{eq:abound-underfit}
\end{align}
using the condition in the Lemma.

\end{proof}

\begin{comment}
\begin{lemma}\label{prop:underestimate}
% Consider $P = Z_0 B Z_0^T$. And $C_1, ..., C_r$ is the true clusters with the normalized clustering matrix $X_0$. $\hat{S}_1, ..., \hat{S}_{\hat{r}}$ is an estimated clusters with cluster size $\hat{r} < r$. Its normalized clustering matrix is $\hat{X}$. If we assume for the true cluster, the cluster size is balanced, i.e., for any $i$, $m_i = |S_i| \geq \pi n = \pi \sum m_i$ for some $\pi$, we can show with high probability $\langle A, \hat{X}\rangle  \leq \langle A, X_0\rangle - \Omega(np_{\text{gap}}),$ where $p_{\text{gap}}= \min_i \min_j B_{i,i} - B_{i,j}$.
% Assume the $\hat{X}^{22}$ in Algorithm \ref{alg:1} satisfies
% $
% \text{trace}(\hat{X}^{22})< r,
% $
% then 
% $\langle A^{22}, \hat{X}^{22}\rangle  \leq \langle A^{22}, X_0^{22}\rangle -\Omega(np_{\text{gap}}\pi_\text{min}^2/r^2)
% $
For any underestimated normalized clustering matrix, i.e., $\text{trace}(\hat{X})< r_0$, if it is independent of $A$, then with high probability ($1-O(1/n)$), $\langle A, \hat{X} \rangle \leq \langle A, X_0 \rangle - \Omega(np_{\text{gap}}\pi_\text{min}^2/r^2)$.
\end{lemma}


\begin{proof}
%We first prove the statement for any network $A$, and a normalized clustering matrix $\hat{X}$ with number of clusters $\hat{r}$, which is independent of $A$.

Based on Lemma~\ref{lem:generalS_under}, we can simply replace $S$ with $P$, and $\tau = n\pi_{\text{min}}p_{\text{gap}}$ where $p_{\text{gap}}=\min_i\min_{j\neq i} B_{i,i}-B_{i,j}$. Then we can obtain 
\begin{equation*}
     \langle P, \hat{X}\rangle \leq \langle P, X_0\rangle- \Omega(np_{\text{gap}}\pi_\text{min}^2/r^2)
\end{equation*}
We then apply Lemma~\ref{lem:generalsamplebound} on both $\langle A-P, \hat{X}\rangle$ and  $\langle A-P, X_0\rangle$, we have with high probability$(1-O(1/n))$, %conditioned on $\hat{X}$ (the training partition),
\begin{equation*}
%\langle A-P, \hat{X}-X_0\rangle \leq 2r \norm{A-P}_2 \leq 2rO(\sqrt{n\rho})
\langle A-P, \hat{X}-X_0\rangle = O_P(\sqrt{r\log n})
\end{equation*}
%by Chernoff, $P(\sum_{i,j\in S_{k}} (A_{ij}-P_{ij}) \leq -cm_k \sqrt{\log n}) \leq 1/n,$
%therefore, $\langle A-P, X_0\rangle \geq - O(r\sqrt{\log n})$ with high probability. 
%Similarly, with high probability, $\langle A-P, \hat{X}\rangle \leq O(\hat{r}\sqrt{\log n}).$

Thus, with high probability. 
\begin{align}
    \langle A, X_0-\hat{X}\rangle &= \langle P, X_0-\hat{X}\rangle - \langle A-P, \hat{X} - X_0\rangle  \nonumber\\
    &= \Omega\left(\frac{np_{gap} {\pi_{\text{min}}^2 }} {r^2}\right) -  O_P(\sqrt{r\log n}) = \Omega\left(\frac{np_{gap} {\pi_{\text{min}}^2 }} {r^2}\right).\label{eq:abound-underfit}
\end{align}

The last line of the above equation is true because of the condition on $p_{\text{gap}}$ in Section~\ref{sec:matrcv_sbm}. 

\end{proof}
\end{comment}


\begin{lemma}\label{prop:overestimate}
% Consider $P = Z_0 B Z_0^T$. And $C_1, ..., C_r$ is the true clusters with the normalized clustering matrix $X_0$. $\hat{S}_1, ..., \hat{S}_{\hat{r}}$ is an estimated clusters with cluster size $\hat{r} < r$. Its normalized clustering matrix is $\hat{X}$. If we assume for the true cluster, the cluster size is balanced, i.e., for any $i$, $m_i = |S_i| \geq \pi n = \pi \sum m_i$ for some $\pi$, we can show with high probability $\langle A, \hat{X}\rangle  \leq \langle A, X_0\rangle - \Omega(np_{\text{gap}}),$ where $p_{\text{gap}}= \min_i \min_j B_{i,i} - B_{i,j}$.
% Assume the $\hat{X}^{22}$ in Algorithm \ref{alg:1} satisfies
% $
% \text{trace}(\hat{X}^{22})< r,
% $
% then 
% $\langle A^{22}, \hat{X}^{22}\rangle  \leq \langle A^{22}, X_0^{22}\rangle -\Omega(np_{\text{gap}}\pi_\text{min}^2/r^2)
% $
For a sequence of overfitting normalized clustering matrix $\{\hat{X}_{r_t}\}_{r<r_t\leq r_T}$, all independent of $A$, $r_T=\Theta(r)$, we have w.h.p. %then with high probability ($1-O(1/n)$), $\langle A, \hat{X} \rangle \leq \langle A, X_0 \rangle + (1+\rho)\sqrt{3\text{trace}(\hat{X})\log n /4}$.
$$
\max_{r<r_t\leq r_T }\langle A, \hat{X}_{r_t} \rangle \leq \langle A, X_0 \rangle + (1+B_{\max})\sqrt{r_T\log n} + B_{\max}r.
$$
\end{lemma}
\begin{proof}
First note, for any $\hat{X}$, using weak assortativity on $B$,
\begin{align}
    \langle P,\hat{X}
    \rangle & \leq \sum_{i,j} \hat{X}_{i,j} B_{C(i), C(j)}  \notag\\
    & \leq \sum_{i} B_{C(i),C(i)}\sum_j \hat{X}_{i,j}   \notag\\
    & \leq \langle P, X_0 \rangle + B_{\max}r,
\end{align}
where $C(i)$ denotes the cluster node $i$ belongs to.
By the same argument as in Eq~\eqref{eq:union_noise}, w.h.p.
\begin{align}
\max_{r<r_t\leq r_T}|\langle A-P, \hat{X}_{r_t} \rangle| \leq (1+B_{\max})\sqrt{r_T\log n}
\label{eq:union_noise_over}
\end{align}

From the above
\begin{align*}
    \max_{r<r_t\leq r_T} \langle A, \hat{X}_{r_t} \rangle &\leq \langle A, X_0 \rangle + (1+B_{\max})\sqrt{r_T\log n} + B_{\max}r. 
\end{align*}

\end{proof}


\begin{lemma}\label{prop:sdp_exactrecovery}
With probabilitiy at least  $1-O(1/n)$, MATR-CV achieves exact recovery on the testing nodes given the true cluster number $r$, i.e. $\hat{X}_r^{22}=X_0^{22}$, provided $n\pi_{\min}\rho / \log n \to \infty$, $\gamma_{\text{train}}=\Theta(1)$.
\end{lemma}

% The above propositions establish that any underfitting normalized clustering matrix $X$ (independent of $A$) will have a significantly smaller $\langle A,X\rangle $ than the ideal value $\langle A,X_0\rangle$. Meanwhile, any overfitting normalized clustering matrix $X$ cannot have a significantly greater $\langle A,X\rangle $ than $\langle A,X_0\rangle$. These two observations indicates that it is possible to find a range of $r$ to exclude all underfitting cases, and ensure including perfect one. Hence, picking the smallest $r$ in the range yields exact recovery, which is the idea of the following model selection algorithm (Algorithm \ref{alg:1}) based on cross-validation.
\begin{proof}
%For the following analysis, we denote $P^{11}$ as the probability matrix for training nodes, $P^{22}$ as the probability matrix for testing nodes. 
Denote $m_k^{11}$, $m_k^{22}$ as the number of nodes belonging to the cluster $C_k$ in the training graph and testing graph respectively. 

First, with Theorem 2 in \cite{yan2017provable} and Lemma~\ref{lem:skala}, we know \ref{SDP:BW} can achieve exact recovery on traininng graph with high probability. Now, consider a node $s$ in testing graph, and assume it belongs to cluster $C_k$. The probability that it is assigned to cluster $k$ is: $P(\frac{\sum_{j\in C_k} A^{21}_{s, j}}{m_k^{11}} \geq \max_{l\neq k}\frac{\sum_{j\in C_l} A^{21}_{s, j}}{m_l^{11}} )$.

Using the Chernoff bound, for some constant $c$,
\begin{align}
    P(\frac{\sum_{j\in C_k} A^{21}_{s, j}}{m_k^{11}} \geq B_{k,k} - c \sqrt{B_{k,k}\log n/m_k^{11}}) \geq 1 - n^{-3};   \notag\\
 P(\frac{\sum_{j\in C_l} A^{21}_{s, j}}{m_l^{11}} \leq B_{l,k} + c \sqrt{B_{l,k}\log n/m_l^{11}}) \geq 1 - n^{-3}.
 \label{eq:chernoff_A12}
\end{align}
Since the graph split is random, for each $k$, with probability at least $1-n^{-3}$, $| m_k^{11}-\gamma_{\text{train}}m_k| \leq c_1\sqrt{m_k\log n}$ for some constant $c_1$. By a union bound, this holds for all $k$ with probability at least $1-rn^{-3}$. Then under this event,
$$
\sqrt{\frac{B_{l,k}\log n}{m_l^{11}}} \leq c_2 \sqrt{\frac{B_{l,k}\log n}{n\pi_{\min}}}
$$
for some $c_2$ since $n\pi_{\min}/\log n \to \infty$. Since $n\pi_{\min}\rho/\log n \to \infty$, by Eq~\eqref{eq:chernoff_A12}, with probabitliy at least $1-O(rn^{-3})$,
$$
B_{k,k} - c \sqrt{B_{k,k}\log n/m_k^{11}} > \max_{l\neq k} B_{l,k} + c \sqrt{B_{l,k}\log n/m_k^{11}},
$$
and node $s$ is assigned correctly to cluster $k$. Taking a union over all $s$ in the training set, with probability 
$1-O(rn^{-2})$, MATR-CV would give exact recovery for the testing graph given $r$.

%Therefore, under the separation condition in the statement of the theorem, $P(\frac{\sum_{j\in S_k} A^{11}_{s, j}}{m_k^{11}} \geq \max_{l\neq k}\frac{\sum_{j\in S_l} A^{11}_{s, j}}{m_l^{11}}  ) \geq 1 - 2r_0n^{-3}$. Then with probability at least $1-2r_0n^{-2}$, with $r_0$ MATR-CV would give exact recovery for testing graph.
\end{proof}


\begin{lemma}\label{lem:skala}
If $m_k\geq \pi n$, then $m_k^{11} \geq \pi n \gamma_\text{train}$, and $m_k^{22}\geq \pi n (1-\gamma_\text{train})$, with high probability.  If $\max_{k,l} \frac{m_k}{m_l}\leq \delta$, then $\max_{k,l} \frac{m^{11}_k}{m^{11}_l} \leq \delta + o(1)$ with high probability.
\end{lemma}
\begin{proof}
The result follows from \cite{skala2013hypergeometric}.
\end{proof}


\noindent{\bf Proof for Theorem~\ref{cor:nok}}
\begin{proof}
First we note that by a similar argument as in Lemma~\ref{prop:sdp_exactrecovery}, $|m_k^{22}-(1-\gamma_{\text{train}})m_k| \leq c\sqrt{m_k \log n}$ for all $k$ with probability at least $1-rn^{-3}$. Then the size of the smallest cluster of the test graph $A^{22}$ will be of the same order as $n\pi_{\text{min}}$. Also $A^{22}$ has size $\Theta(n)$. $A^{22}$ is independent of any $\hat{X}^{22}$. Thus in Theorem~\ref{thm:matrcv_general}, applying Lemma~\ref{prop:underestimate} and Lemma~\ref{prop:overestimate} to $A^{22}$ shows
$$
\epsilon_{under}= \Omega(n\rho \pi_{\text{min}}^2 /r^2),
$$
$$
\epsilon_{over}= (1+B_{\max})\sqrt{r_T\log n} + B_{\max}r,
$$
and Lemma~\ref{prop:sdp_exactrecovery} shows $\epsilon_{est}=0$, w.h.p. For fixed $r, \pi_{\min}$, we have $\epsilon_{under} \gg \epsilon_{over}$.
By Theorem~\ref{thm:matrcv_general}, choosing
$\Delta=(1+B_{\max}) \sqrt{r_T\log n}+B_{\max}r$ leads to MATR-CV returning the correct $r$. We can further refine $\Delta$ by noting that $
    r_{\max}:=\arg\max_{r_t}\langle A, \hat{X}_{r_t} \rangle \geq r
    $ w.h.p., then it suffices to consider the candidate range $\{r_1, \dots, r_{\max}\}$. The same arguments still hold for this range, thus $r_T$ and $r$ in $\Delta$ can be replaced with $r_{\max}$.
\end{proof}

\subsection{Proof of Theorem~\ref{thm:nok_mmsb}}

 
In the following, we show theoretical guarantees of using MATR-CV to do model selection on MMSB with the SPACL algorithm proposed by \cite{Mao2017EstimatingMM}. We assume $A$ has self-loops for clarify of exposition. Adding the diagonal terms introduces a term that is asymptotically negligible compared with other terms, thus does not change our results. 


First we have the following concentration lemma regarding the criterion $\langle A^2-\text{diag}(A^2), X \rangle$ for a general normalized clustering matrix $X$, which will be used to derive the three errors in Theorem~\ref{thm:matrcv_general}.

\begin{lemma}
For any general normalized clustering matrix $X$ satisfying $X\mathbf{1}_n=\mathbf{1}_n$, and an adjacency matrix $A$ generated from its expectation matrix $P$ independent of $X$, w.h.p.
\begin{align}
    \langle \hat{S}-S, X\rangle = O(n\rho\sqrt{\log n}),
\end{align}
where $\hat{S}=A^2-\text{diag}(A^2)$, $S=P^2-\text{diag}(P^2)$.
\label{lem:A2_conc}
\end{lemma}

\begin{proof}

\begin{align}
\langle \hat{S}-S, X\rangle&=\sum_{j, i\neq k}(A_{ij}A_{jk}-P_{ij}P_{jk})X_{ik}\notag\\
&=\underbrace{\sum_{i,j,k}(A_{ij}A_{jk}-E[A_{ij}A_{jk}])X_{ik}}_{\text{Part (i)}}-\underbrace{\sum_{i,j}(A_{ij}-E[A_{ij}])X_{ij}}_{\text{Part (ii)}}
\label{eq:part1part2_A2}
\end{align}

To bound Part (i), we will first bound $f(A_{ij},1\leq i\le j \leq n)=\sum_{i,j,k}A_{ij}A_{jk}X_{ik}/2$.  Let
\begin{align*}
f_{uv}:=f(A_{ij},1\leq i\le j \leq n, A_{uv}=0)=f(A)-\frac{A_{uv}\sum_{k}A_{vk}X_{uk}+A_{uv}\sum_{i}A_{iu}X_{iv}}{2},
\end{align*}
%and $\tilde{d}_{u,\ell}$ denote $d_{u,\ell}-A_{uv}$. 
Clearly, $0\leq f-f_{uv}\leq 1$ since $X\mathbf{1}_n=\mathbf{1}_n$, and 
\begin{align*}
\sum_{u<v} (f-f_{uv})&\leq \sum_{u<v}\frac{A_{uv}\sum_{k}A_{vk}X_{uk}+A_{uv}\sum_{i}A_{iu}X_{iv}}{2}\\
&\leq \frac{1}{2}\sum_{u,v}\frac{A_{uv}\sum_{k}A_{vk}X_{uk}+A_{uv}\sum_{i}A_{iu}X_{iv}}{2}\\
&\leq \frac{1}{2}\sum_{u,v,k}\frac{A_{uv}A_{vk}X_{uk}+A_{iu}A_{uv}X_{iv}}{2}\\
&\leq f/2
\end{align*}
So $f$ is $(1/2,0)$ self bounding. Hence,
\begin{align*}
P(f-E[f]\geq t)\leq \exp\left(\frac{-t^2}{E[f]+t}\right)\\
P(f-E[f]\leq -t)\leq \exp\left(\frac{-t^2}{E[f]+2t/3}\right)
\end{align*}
Note that $E[f]=\Theta(n^2\rho^2)$, and so setting $t=\Theta(n\rho\sqrt{\log n})$ we get:
\begin{align*}
P(f-E[f]\geq t)= O(1/n)\\
P(f-E[f]\leq -t)=O(1/n)
\end{align*}

Using the same argument on Part (ii), shows that it is $O(\sqrt{n\rho\log n})$ w.h.p.


Therefore using Eq~\eqref{eq:part1part2_A2}, we see that:
\begin{align*}
\langle \hat{S}-S,X\rangle =O(n\rho\sqrt{\log n})
\end{align*}
w.h.p.
\end{proof}

The next two propositions are for general underfitting and overfitting normalized clustering matrices $\hat{X}$ independent of $A$, which will be used to derive $\epsilon_{\text{under}}$ and $\epsilon_{\text{over}}$.

%Cnd consider the singular value decomposition of $\Theta = U D V^T$($U$ is rectangular), and $\hat {\Theta} = \hat{U} \hat{D} \hat{V}^T$. Then $\hat{X} = \hat{\Theta} (\hat{\Theta} ^T \hat{\Theta})^{-1} \hat{\Theta}^T = \hat{U}\hat{U}^T,$ and $\Theta \Theta^T = UD^2U^T.$

\begin{Proposition}\label{prop:underestimatemmsb}
For a sequence of underfitting normalized clustering matrix $\{\hat{X}_{r_t}\}_{r_t<r}$, all independent of $A$, then with high probability, $\max_{r_t<r}\langle A^2-\text{diag}(A^2), \hat{X}_{r_t} \rangle \leq \langle A^2-\text{diag}(A^2), X_0 \rangle - \Omega(n^2\rho^2)$.
\end{Proposition}

\begin{proof}
Suppose $P=\Theta B \Theta^T$ has eigenvalue decomposition $Q\Lambda Q^T$. Also consider the singular value decomposition of $\hat {\Theta} = \hat{U} \hat{D} \hat{V}^T$, then $\hat{X}_{r_t} = \hat{\Theta} (\hat{\Theta} ^T \hat{\Theta})^{-1} \hat{\Theta}^T = \hat{U}\hat{U}^T$.  We have
%\rd (form of $P$ is used here)\bk
\begin{align}
\langle P^2, X_0 - \hat{X}_{r_t} \rangle & = \tr{P^2} - \tr{P^2\hat{U}\hat{U}^T}    \notag\\
& = \tr{\Lambda^2} - \tr{\Lambda^2Q^T \hat{U}\hat{U}^T Q}  \notag\\
& = \tr{\Lambda^2} - \tr{\Lambda^2\hat{Q}^T \hat{Q}} \notag\\
& \geq \min_{i}\Lambda_{i,i}^2 =  (\lambda^*(P))^2,  
\label{eq:mmsb_under_pop}
\end{align}
where $\hat{Q}:= \hat{U}^T Q$, $\lambda^*(P)$ is the smallest singular value of $P$. The last line follows from Von Neumann's trace inequality and the fact that $\norm{\hat{Q}^T\hat{Q}}_{op} \leq 1$ and $\text{rank}(\hat{Q}^T\hat{Q})\leq r_t<r$.

Applying Lemma B.4 and Lemma 3.6 in \cite{Mao2017EstimatingMM} to \eqref{eq:mmsb_under_pop}, with probability at least $1-r_0\exp\left(-\frac{n}{36\nu^2(1+\alpha_0)^2}\right)$, 
\begin{align}
    \langle P^2, X_0 - \hat{X}_{r_t} \rangle \geq \frac{n^2(\lambda^*(B))^2}{4\nu^2(1+\alpha_0)^2},
\end{align}
that is, $\langle P^2, X_0 - \hat{X}_{r_t} \rangle = \Omega_P(n^2\rho^2)$.

Now 
\begin{align}
    |\langle \text{diag}(P^2), X_0 - \hat{X}_{r_t} \rangle | \leq 2\max_i(P^2)_{ii}\tr{X_0} = O(n\rho^2).
    \label{eq:diagP2}
\end{align}
By Lemma~\ref{lem:A2_conc}, with a union bound since $r$ is fixed,
$$
\max_{r_t<r} |\langle \hat{S} -S, \hat{X}_{r_t} \rangle| = O_P(n\rho\sqrt{\log n})
$$
We have the desired inequality. 

%Noting that $A^2-P^2 = (A-P)^2+P(A-P)+(A-P)P$, 
%\begin{align} 
%| \langle
%(A-P)^2, \hat{X}_k - X_0
%\rangle | \leq 2\|(A-P)^2\|_{op} \tr{X_0} = O(n\rho)
%\label{eq:mmsb_under_noise1}
%\end{align}
%with probability at least $1-n^{-1}$. By Lemma~\ref{lem:generalsamplebound}, since $\hat{X}_k$ and $A$ are independent, 
%\begin{align}
%   | \langle
%A-P, P(\hat{X}_k - X_0)
%\rangle | = O(\sqrt{\tr{PX_0} \log n}) = O(\sqrt{n\rho \log n})
%\label{eq:mmsb_under_noise2}
%\end{align}
%with probability at least $1-O(n^{-1})$. Here we use the fact that $\tr{PX_0} \leq \|P\|_F \tr{X_0}=O(n\rho)$. Finally,
%\begin{align}
%   |\langle diag(A^2), \hat{X}_k - X_0 \rangle | & \leq 2 \max_i (A^2)_{i,i} \tr{X_0} \notag\\
%   & = 2r_0 \max_i \sum_k A_{i,k} \notag\\
%   & = 2r_0 \max_i \sum_k [(A_{i,k}-P_{i,k}) + P_{i,k}]    \notag\\
%   & = O(\sqrt{n\rho}\log n) + O(n\rho) = O(n\rho)
%   \label{eq:mmsb_under_noise3}
%\end{align}
%w.h.p., since $\max_i\sum_k (A_{i,k}-P_{i,k})=O(\sqrt{n\rho}\log n)$ w.h.p., and $\sqrt{n\rho}/\log n \to \infty$.
%\rd Also shouldnt the above have trace of $\hat{X}_k$ as well?\bk
%Eqs~\eqref{eq:mmsb_under_noise1}-\eqref{eq:mmsb_under_noise3} imply w.h.p. 
%\begin{align}
%    |\langle A^2-P^2-diag(A^2), \hat{X}_k - X_0\rangle| = O(n\rho),
%\end{align}
%and $\langle A^2 -diag(A^2), X_0-\hat{X}_k \rangle = \Omega(n^2\rho^2)$ w.h.p.


\end{proof}







\begin{Proposition}\label{prop:overestimatemmsb}
% Aonsider $P = Z_0 B Z_0^T$. And $C_1, ..., C_r$ is the true clusters with the normalized clustering matrix $X_0$. $\hat{S}_1, ..., \hat{S}_{\hat{r}}$ is an estimated clusters with cluster size $\hat{r} < r$. Its normalized clustering matrix is $\hat{X}$. If we assume for the true cluster, the cluster size is balanced, i.e., for any $i$, $m_i = |S_i| \geq \pi n = \pi \sum m_i$ for some $\pi$, we can show with high probability $\langle A, \hat{X}\rangle  \leq \langle A, X_0\rangle - \Omega(np_{\text{gap}}),$ where $p_{\text{gap}}= \min_i \min_j B_{i,i} - B_{i,j}$.
% Cssume the $\hat{X}^{22}$ in Clgorithm \ref{alg:1} satisfies
% $
% \text{trace}(\hat{X}^{22})< r,
% $
% then 
% $\langle A^{22}, \hat{X}^{22}\rangle  \leq \langle A^{22}, X_0^{22}\rangle -\Omega(np_{\text{gap}}\pi_\text{min}^2/r^2)
% $
For a sequence of overfitting normalized clustering matrix $\{\hat{X}_{r_t}\}_{r<r_t\leq r_T}$ independent of $A$, with high probability, $$\max_{r<r_t\leq r_T}\langle A^2-\text{diag}(A^2), \hat{X}_{r_t} \rangle \leq \langle A^2-\text{diag}(A^2), X_0 \rangle + O(n\rho \sqrt{\log n})$$.
\end{Proposition}

\begin{proof}
First note by a similar argument as~\eqref{eq:mmsb_under_pop}, %(\rd this may need modification for deg corrected \bk)
\begin{align}
   \langle P^2, X_0 - \hat{X}_{r_t} \rangle = \tr{\Lambda^2} - \tr{\Lambda^2 \hat{Q}^T\hat{Q}} \geq 0.
\end{align}
Since $\hat{X}_{r_t}$ and $A$ are independent, by an argument similar to~\eqref{eq:diagP2} and Lemma~\ref{lem:A2_conc}, 
\begin{align}
   \max_{r<r_t\leq r_T}\langle A^2-\text{diag}(A^2), \hat{X}_{r_t} \rangle \leq \langle A^2-\text{diag}(A^2), X_0 \rangle + O(n\rho\sqrt{\log n})
\end{align}
w.h.p.
\end{proof}

Next we derive the estimation error by considering the parameter estimates recovered by SPACL \citep{Mao2017EstimatingMM}. For notational convenience, we first derive some bounds for $\hat{\Theta}$ and $\hat{B}$ estimated from the matrix $A$, with the understanding that the same asymptotic bounds apply to estimates obtained from the training graph provided the split is random and the number of training nodes is $\Theta(n)$. The next lemma states the parameter estimation error from \cite{Mao2017EstimatingMM}. 

%\rd update for dcmmsb \bk
\begin{lemma}
There exists a permutation matrix $\Pi$, such that, with probability larger than $1-O(rn^{-2})$,
\begin{align}
    \Delta_1 & := \norm{\hat{\Theta}-\Theta\Pi}_F = O\left(\frac{(\log n)^{1+\xi}}{\sqrt{\rho}}\right),  \label{eq:thetabound}  \\
    \Delta_2 &:= \norm{\hat{B}- \Pi ^T B \Pi}_F = O(\sqrt{\frac{\rho}{n}} (\log n)^{1+\xi}).
\end{align}

\label{lem:mmsb_para_error} 
\end{lemma}

\begin{proof}
These bounds follow directly from Corollary 3.7 of \cite{Mao2017EstimatingMM}, with $\alphav, r, \lambda^*(B/\rho)$ all being constant.
\end{proof}

%Suppose $B = \rho B_0$. From the proof of Theorem 3.5 in \cite{Mao2017EstimatingMM}, we know that there exists a permutation matrix $\Pi$, such that, with probability larger than $1-O(Kn^{-2})$,
%\begin{equation}\label{eq:thetabound}
%    \norm{\ev_i^T(\hat{\Theta} - \Theta \Pi)} \leq \tilde{O}(\frac{r_0^3 \nu ^3 (1+\alpha_0)^2}{\sqrt{\rho n} \lambda^*(B_0)}),
%\end{equation}
%\begin{equation}\label{eq:bbound}
%    \norm{\hat{B}- \Pi ^T B \Pi}_F \leq \tilde{O}(\frac{r_0^3\nu^3 (1+\alpha_0)^2\sqrt{\rho}}{\sqrt{ n } \lambda ^*(B_0)}).
%\end{equation}

In what follows, we omit the permutation matrix $\Pi$ to simplify notation. If $\Pi$ is not the identity matrix, we can always redefine $\Theta$ as $\Theta \Pi$, and $B$ as $\Pi^TB \Pi$. This would not affect the results, since we want to prove bounds on normalized clustering matrices where $\Pi$ always cancels out, i.e., $X = \Theta \Pi ((\Theta \Pi)^T \Theta \Pi)^{-1}(\Theta \Pi)^T = \Theta (\Theta^T \Theta)^{-1}\Theta^T.$


We are interested in bounding the estimation error in $\hat{H}=\hat{B}^{-1}(\hat{\Theta}^T\hat{\Theta})^{-1}\hat{\Theta}^T$. In order to build up the bound, we will make repeated use of the following two facts.

\begin{fact}\label{lem:prodminus}
For general matrices $C, \hat{C}, D, \hat{D}$,
$$\norm{\hat{C}\hat{D} - CD}_F \leq \norm{(\hat{C}-C)(\hat{D}-D)}_F + \norm{(\hat{C}-C)D}_F + \norm{C(\hat{D}-D)}_F$$
\end{fact}

\begin{proof}
The proof follows directly from expansion and the triangle inequality,
$$\hat{C}\hat{D} - CD = (\hat{C}-C)(\hat{D}-D) + (\hat{C}-C)D + C(\hat{D}-D).$$

\end{proof}


\begin{fact}
\label{lem:invminus}
For a general matrices $C$, $\hat{C}$, assume $\norm{(C-\hat{C})C^{-1}}_F< 1$, then 
$$\norm{\hat{C}^{-1} - C^{-1}}_F \leq \frac{\norm{C^{-1}}_F \norm{(C-\hat{C}) C^{-1}}_F}{1- \norm{(C-\hat{C})C^{-1}}_F}$$
\end{fact}
\begin{proof}
First decompose
\begin{align}
    \hat{C}^{-1}-C^{-1} = \hat{C}^{-1}CC^{-1} - C^{-1}=(\hat{C}^{-1}C-I)C^{-1}=\hat{C}^{-1}(C-\hat{C}) C^{-1}.
    \label{eq:invminus_decomp}
\end{align}
Taking Frobenius norms,
$$\norm{\hat{C}^{-1}}_F \leq \norm{C^{-1}}_F + \norm{\hat{C}^{-1} (C-\hat{C})C^{-1}}_F \leq \norm{C^{-1}}_F + \norm{\hat{C}^{-1}}_F \norm{(C-\hat{C})C^{-1}}_F .$$
Rearranging, 
$$\norm{\hat{C}^{-1}}_F\leq \frac{\norm{C^{-1}}_F}{1- \norm{(C-\hat{C}) C^{-1}}_F}.$$
Applying this to~\eqref{eq:invminus_decomp},
$$\norm{\hat{C}^{-1} -C^{-1}}_F\leq \norm{\hat{C}^{-1}}_F \norm{(C-\hat{C}) C^{-1}}_F \leq \frac{\norm{C^{-1}}_F \norm{(C-\hat{C}) C^{-1}}_F}{1- \norm{(C-\hat{C}) C^{-1}}_F}.$$
\end{proof}

Next we have a lemma bounding the error in estimating the quantity $H = B^{-1}(\Theta^T\Theta)^{-1}\Theta^T$.

\begin{lemma}
Let $H = B^{-1}(\Theta^T\Theta)^{-1}\Theta^T$, $\hat{H} = \hat{B}^{-1}(\hat{\Theta}^T\hat{\Theta})^{-1}\hat{\Theta}^T$, then w.h.p.
\begin{align}
    \norm{H-\hat{H}}_F = O\left( \frac{(\log n)^{1+\xi}}{n\rho^{3/2}}\right)   \notag\\
    \norm{H}_F=O\left(\frac{1}{\sqrt{n}\rho}. \right)
\end{align}
% $$\norm{G-\hat{G}}_F \leq 2\Delta_2 F_2^2F_1+ 2F_2((\Delta_1^2 + 2\sqrt{n} \Delta_1)F_1^2), $$

% $$\norm{G}_F\leq 2 F_2\nu (1+\alpha_0)/n,$$
%$$\norm{H-\hat{H}}_F \leq \sqrt{n} \Delta_3 + (F_1F_2+ \Delta_3) \Delta_1,$$
%$$\norm{H}_F\leq 2 F_2\nu (1+\alpha_0)/\sqrt{n},$$
%where $\Delta_3 = 2\Delta_2 F_2^2F_1+ 2F_2((\Delta_1^2 + 2\sqrt{n} \Delta_1)F_1^2).$
\label{lem:Hhat}
\end{lemma}

\begin{proof}
We build up the estimator of $H$ step by step by repeatedly using Facts~\ref{lem:prodminus} and \ref{lem:invminus}. Denote $F_1=\norm{(\Theta^T\Theta)^{-1}}_F$, and $F_2 = \norm{B^{-1}}_F$, by Lemma 3.6 in \cite{Mao2017EstimatingMM}, 
\begin{align}
 F_1 \leq \sqrt{r_0} \norm{(\Theta^T\Theta)^{-1}}_{op} = O_P(1/n),    \label{eq:fnorm_F1}
\end{align}
and 
\begin{align}
    F_2 \leq \sqrt{r}\norm{B^{-1}}_{op} = O(1/\rho).
    \label{eq:fnorm_F2}
\end{align}

First, applying Fact~\ref{lem:prodminus}, 
\begin{align*}
    \norm{\hat{\Theta}^T\hat{\Theta} - \Theta ^T \Theta}_F &\leq \Delta_1^2 + 2\norm{\Theta}_{F} \Delta_1    \\
    \norm{(\Theta ^T \Theta)^{-1}}_F \norm{\hat{\Theta}^T\hat{\Theta} - \Theta ^T \Theta}_F & \leq (\Delta_1^2 + 2\norm{\Theta}_{F} \Delta_1)F_1    \\
    & = O_P\left(\frac{(\log n)^{2+2\xi}}{n\rho}\right) + O_P\left( \frac{(\log n)^{1+\xi}}{\sqrt{n\rho}}   \right) \\
    & = O_P\left( \frac{(\log n)^{1+\xi}}{\sqrt{n\rho}}   \right),
\end{align*}
using Lemma \ref{lem:mmsb_para_error} and eq~\eqref{eq:fnorm_F1}. Thus for large $n$, $\norm{(\Theta ^T \Theta)^{-1}}_F \norm{\hat{\Theta}^T\hat{\Theta} - \Theta ^T \Theta}_F<1/2$.  Then using Fact~\ref{lem:invminus}, we have 
\begin{align}
    \norm{(\hat{\Theta}^T\hat{\Theta})^{-1} - (\Theta^T\Theta)^{-1}}_F &\leq \frac{\norm{(\Theta^T\Theta)^{-1}}_F \norm{((\Theta^T\Theta)-(\hat{\Theta}^T\hat{\Theta})) (\Theta^T\Theta)^{-1}}_F}{1- \norm{((\Theta^T\Theta)-(\hat{\Theta}^T\hat{\Theta}))(\Theta^T\Theta)^{-1}}_F} \notag\\
    & \leq \frac{\norm{(\Theta^T\Theta)^{-1}}_F^2 \norm{((\Theta^T\Theta)-(\hat{\Theta}^T\hat{\Theta}))}_F}{1- \norm{((\Theta^T\Theta)-(\hat{\Theta}^T\hat{\Theta}))(\Theta^T\Theta)^{-1}}_F} \notag\\
    % & \leq \frac{\norm{(\Theta^T\Theta)^{-1}}_F^2 (\norm{\hat{\Theta} - \Theta}_F^2 + 2 \norm{\Theta^T(\hat{\Theta} - \Theta)}_F)}{1- \norm{((\Theta^T\Theta)-(\hat{\Theta}^T\hat{\Theta}))(\Theta^T\Theta)^{-1}}_F}\\
    & \leq 2\norm{(\Theta^T\Theta)^{-1}}_F^2 \norm{((\Theta^T\Theta)-(\hat{\Theta}^T\hat{\Theta}))}_F \notag\\
    % & \leq  \frac{F_1^2 (\Delta_1^2 + 2\norm{\Theta}_F \Delta_1)}{1- F_1 (\Delta_1^2+ 2\norm{\Theta}_F \Delta_1)}\\
    & \leq (\Delta_1^2 + 2\norm{\Theta}_{F} \Delta_1)F_1^2 = O_P\left(\frac{(\log n )^{1+\xi}}{n^{3/2}\rho^{1/2}}.
    \label{eq:thetainv_error}
    \right)
\end{align} 

Similarly using Lemma~\ref{lem:mmsb_para_error} and eq~\eqref{eq:fnorm_F2}, by noting that $$\norm{B^{-1}}_F\norm{(B-\hat{B})}_F = \Delta_2 F_2 = O(\frac{(\log n)^{1+\xi}}{\sqrt{n\rho}})< 1/2$$ for large $n$ w.h.p.,
\begin{align}
    \norm{\hat{B}^{-1} - B^{-1}}_F &\leq  \frac{\norm{B^{-1}}_F \norm{(B-\hat{B}) B^{-1}}_F}{1- \norm{(B-\hat{B})B^{-1}}_F}    \notag\\
    & \leq 2 \norm{B^{-1}}_F^2\norm{(B-\hat{B})}_F \notag\\
    % & \leq \frac{\norm{(\Theta^T\Theta)^{-1}}_F^2 (\norm{\hat{\Theta} - \Theta}_F^2 + 2 \norm{\Theta^T(\hat{\Theta} - \Theta)}_F)}{1- \norm{((\Theta^T\Theta)-(\hat{\Theta}^T\hat{\Theta}))(\Theta^T\Theta)^{-1}}_F}\\
    & \leq 2\Delta_2 F_2^2 = O_P\left( \frac{(\log n)^{1+\xi}}{n^{1/2}\rho^{3/2}}\right)
    \label{eq:Binv_error}
\end{align}
using Fact~\ref{lem:invminus}.

Next applying Fact~\ref{lem:prodminus} to $G := B^{-1}(\Theta^T\Theta)^{-1}$ and its estimate $\hat{G} := \hat{B}^{-1}(\hat{\Theta}^T\hat{\Theta})^{-1}$,

\begin{align*}
& \norm{G - \hat{G}}_F  \notag\\
  \leq & \norm{\hat{B}^{-1} - B^{-1}}_F F_1 +
 (\norm{B^{-1}}_F+ \norm{B^{-1}- \hat{B}^{-1}}_F)\norm{(\hat{\Theta}^T\hat{\Theta})^{-1} - (\Theta^T\Theta)^{-1}}_F \\
 \leq & 2\Delta_2 F_2^2F_1+ (2\Delta_2 F_2^2 + F_2)(\Delta_1^2 + 2\norm{\Theta}_{F} \Delta_1)F_1^2 \notag\\
= & O_P\left( \frac{(\log n)^{1+\xi}}{(n\rho)^{3/2}}\right), 
\end{align*}
 using Eqs~\eqref{eq:fnorm_F1}-\eqref{eq:Binv_error}.

Finally, since $H = G\Theta^T$, and $\hat{H} = \hat{G}\hat{\Theta}^T$, 
\begin{align*}
    \norm{H-\hat{H}}_F & \leq \norm{\hat{G} - G}_F \norm{\Theta}_{F} + (\norm{G}_F+ \norm{G- \hat{G}}_F)\norm{\hat{\Theta}-\Theta}_F \\
    & \leq \sqrt{n} \norm{G - \hat{G}}_F + (F_1F_2+ \norm{G - \hat{G}}_F) \Delta_1    \\
    & = O_P\left( \frac{(\log n)^{1+\xi}}{n\rho^{3/2}}\right),
\end{align*}
and 
\begin{align*}
    \norm{G}_F^2 & = \text{tr} ((\Theta^T\Theta)^{-1}(\Theta^T\Theta)^{-1} (BB^T)^{-1})\\
    & \leq \norm{(\Theta^T\Theta)^{-1}}_{op}^2 \text{tr}((BB^T)^{-1})\\
    & = O_P(1/n^2) F_2^2
\end{align*}
 by Eq~\eqref{eq:fnorm_F1},
$\norm{H}_F=O_P(\frac{1}{\sqrt{n}\rho})$ follows.
\end{proof}









%\begin{lemma}
%Consider the $\hat{\Theta}$ and $\hat{B}$ from SPCCL, then 
%$$\norm{(\hat{\Theta}^T\hat{\Theta})^{-1} - (\Theta^T\Theta)^{-1}}_F \leq  (\Delta_1^2 + 2\norm{\Theta}_{F} \Delta_1)F_1^2,$$
%$$\norm{\hat{B}^{-1} - B^{-1}}_F\leq 2\Delta_2 F_2^2.$$
%\end{lemma}


% \begin{lemma}
% Consider the $\hat{\Theta}$ and $\hat{B}$ from SPCCL, then 
% $$\norm{(\hat{\Theta}^T\hat{\Theta})^{-1} - (\Theta^T\Theta)^{-1}}_F \leq \tilde{O}(\frac{r_0^{8} \nu ^8 (1+\alpha_0)^6}{\sqrt{\rho} \lambda^*(B_0)n^{1.5}}),$$
% $$\norm{\hat{B}^{-1} - B^{-1}}_F\leq \tilde{O}(\frac{r_0^{4}\nu^3 (1+\alpha_0)^2}{\sqrt{ n}\rho^{1.5} \lambda ^*(B_0)^3})).$$
% \end{lemma}

% \begin{proof}



% First, with Lemma~\ref{lem:prodminus}, 
% \begin{align*}
%     \norm{\hat{\Theta}^T\hat{\Theta} - \Theta ^T \Theta}_F &\leq \Delta_1^2 + 2\norm{\Theta}_{F} \Delta_1\\
%     &\leq \tilde{O}(\frac{r_0^6 \nu ^6 (1+\alpha_0)^4}{\rho \lambda^{*}(B_0)^2}) + \tilde{O}(\frac{r_0^3 \nu ^3 (1+\alpha_0)^2\sqrt{n}}{\sqrt{\rho} \lambda^*(B_0)})\\
%     &\leq \tilde{O}(\frac{r_0^6 \nu ^6 (1+\alpha_0)^4\sqrt{n}}{\sqrt{\rho} \lambda^*(B_0)})
% \end{align*}

% \xj{how to add two order.}
% Therefore,
% $$\norm{(\Theta ^T \Theta)^{-1}}_F \norm{\hat{\Theta}^T\hat{\Theta} - \Theta ^T \Theta}_F \leq \tilde{O}(\frac{r_0^{7.5} \nu ^7 (1+\alpha_0)^5}{\sqrt{\rho n} \lambda^*(B_0)}).$$

% When $n$ is large, $\norm{(\Theta ^T \Theta)^{-1}}_F \norm{\hat{\Theta}^T\hat{\Theta} - \Theta ^T \Theta}_F<1$, then use Lemma~\ref{lem:invminus}, we have 
% \begin{align*}
%     \norm{(\hat{\Theta}^T\hat{\Theta})^{-1} - (\Theta^T\Theta)^{-1}}_F &\leq \frac{\norm{(\Theta^T\Theta)^{-1}}_F \norm{((\Theta^T\Theta)-(\hat{\Theta}^T\hat{\Theta})) (\Theta^T\Theta)^{-1}}_F}{1- \norm{((\Theta^T\Theta)-(\hat{\Theta}^T\hat{\Theta}))(\Theta^T\Theta)^{-1}}_F}\\
%     & \leq \frac{\norm{(\Theta^T\Theta)^{-1}}_F^2 \norm{((\Theta^T\Theta)-(\hat{\Theta}^T\hat{\Theta}))}_F}{1- \norm{((\Theta^T\Theta)-(\hat{\Theta}^T\hat{\Theta}))(\Theta^T\Theta)^{-1}}_F}\\
%     % & \leq \frac{\norm{(\Theta^T\Theta)^{-1}}_F^2 (\norm{\hat{\Theta} - \Theta}_F^2 + 2 \norm{\Theta^T(\hat{\Theta} - \Theta)}_F)}{1- \norm{((\Theta^T\Theta)-(\hat{\Theta}^T\hat{\Theta}))(\Theta^T\Theta)^{-1}}_F}\\
%     & \leq 2\norm{(\Theta^T\Theta)^{-1}}_F^2 \norm{((\Theta^T\Theta)-(\hat{\Theta}^T\hat{\Theta}))}_F\\
%     % & \leq  \frac{F_1^2 (\Delta_1^2 + 2\norm{\Theta}_F \Delta_1)}{1- F_1 (\Delta_1^2+ 2\norm{\Theta}_F \Delta_1)}\\
%     & \leq \tilde{O}(\frac{r_0^{8} \nu ^8 (1+\alpha_0)^6}{\sqrt{\rho} \lambda^*(B_0)n^{1.5}})
% \end{align*}

% Similarly, for $B$ and $\hat{B}$, $\norm{B^{-1}}_F \leq \sqrt{r_0}\norm{B^{-1}}_{op} \leq O(\frac{\sqrt{r_0}}{\rho \lambda^*(B_0)}),$ 

% so
% $$\norm{B^{-1}}_F\norm{(B-\hat{B})}_F\leq \tilde{O}(\frac{r_0^{3.5}\nu^3 (1+\alpha_0)^2}{\sqrt{ n \rho} \lambda ^*(B_0)^2}))< 1, \text{when $n$ is large}.$$
% With Lemma~\ref{lem:invminus}, we have, 

% \begin{align*}
%     \norm{\hat{B}^{-1} - B^{-1}}_F &\leq  \frac{\norm{B^{-1}}_F \norm{(B-\hat{B}) B^{-1}}_F}{1- \norm{(B-\hat{B})B^{-1}}_F}\\
%     & \leq 2 \norm{B^{-1}}_F^2\norm{(B-\hat{B})}_F\\
%     % & \leq \frac{\norm{(\Theta^T\Theta)^{-1}}_F^2 (\norm{\hat{\Theta} - \Theta}_F^2 + 2 \norm{\Theta^T(\hat{\Theta} - \Theta)}_F)}{1- \norm{((\Theta^T\Theta)-(\hat{\Theta}^T\hat{\Theta}))(\Theta^T\Theta)^{-1}}_F}\\
%     & \leq \tilde{O}(\frac{r_0^{4}\nu^3 (1+\alpha_0)^2}{\sqrt{ n}\rho^{1.5} \lambda ^*(B_0)^3})).
% \end{align*}




% \end{proof}


\begin{lemma}Consider applying SPACL on the training graph $A^{11}$ to obtain $(\hat{\Theta}^{11})^T$ and $\hat{B}$, and use regression in MATR-CV to estimate membership matrix, i.e., $(\hat{\Theta}^{22})^T = \hat{B}^{-1}((\hat{\Theta}^{11})^T\hat{\Theta}^{11})^{-1}(\hat{\Theta}^{11})^T A^{12}:= \hat{H}A^{12}$, then $\norm{\hat{\Theta}^{22} - \Theta^{22}}_F = O\left( \frac{(\log n)^{1+\xi}}{\sqrt{\rho}}\right) $ w.h.p.
\label{lem:theta_est_error}
\end{lemma}

\begin{proof}
Since $(\Theta^{22})^T =H\Theta^{11}B(\Theta^{22})^T$, where $H :={B}^{-1}((\Theta^{11})^T{\Theta}^{11})^{-1}(\Theta^{11})^T$,  
\begin{equation*}
\begin{aligned}
    (\hat{\Theta}^{22})^T-(\Theta^{22})^T &= \hat{H}{A}^{12}-H\Theta^{11}B(\Theta^{22})^T\\
    &=\hat{H}{A}^{12}-\hat{H}\Theta^{11}B(\Theta^{22})^T+\hat{H}\Theta^{11}B(\Theta^{22})^T-H\Theta^{11}B(\Theta^{22})^T\\
    &=\hat{H}(A^{12}-\Theta^{11}B(\Theta^{22})^T)+(\hat{H}-H)\Theta^{11}B(\Theta^{22})^T\\
    &= \underbrace{H(A^{12}-P^{12})}_{Q_1}+\underbrace{(\hat{H}-H)(A^{12}-P^{12})}_{Q_2}+\underbrace{(\hat{H}-H)P^{12}}_{Q_3}.
\end{aligned}
\end{equation*}
For $Q_1$, 
\begin{align*}
    \norm{Q_1}_F &\leq \norm{A^{12}-P^{12}}_{op} \norm{H}_F\\  %= O(\sqrt{n\rho})\norm{H}_F\\
    &= O_P(\sqrt{n\rho})O_P(\frac{1}{\sqrt{n}\rho}) = O_P(1/\sqrt{\rho})
\end{align*}
by Lemma~\ref{lem:Hhat}. For $Q_2$,
\begin{align*}
    \norm{Q_2}_F &\leq \norm{A^{12}-P^{12}}_{op} \norm{\hat{H}-H}_F\\  %= O(\sqrt{n\rho})\norm{H}_F\\
    &= O_P(\sqrt{n\rho})O_P\left( \frac{(\log n)^{1+\xi}}{n\rho^{3/2}}\right) = O_P\left( \frac{(\log n)^{1+\xi}}{\sqrt{n}\rho}\right),
\end{align*}
 by Lemma~\ref{lem:Hhat}. Finally for $Q_3$, 
\begin{align*}
    \norm{Q_3}_F &\leq \norm{P^{12}}_{F} \norm{\hat{H}-H}_F\\  %= O(\sqrt{n\rho})\norm{H}_F\\
    &= O_P(n\rho)O_P\left( \frac{(\log n)^{1+\xi}}{n\rho^{3/2}}\right) = O_P\left( \frac{(\log n)^{1+\xi}}{\sqrt{\rho}}\right),
\end{align*}
The above arguments lead to

\begin{align*}
    \norm{\hat{\Theta}^{22} - \Theta^{22}}_F %& \leq O(\sqrt{n\rho})F_2\nu (1+\alpha_0)/n +\\
    %& O(n\rho)\{\sqrt{n} \Delta_3 + (F_1F_2+ \Delta_3) \Delta_1\}
    = O_P\left( \frac{(\log n)^{1+\xi}}{\sqrt{\rho}}\right).
\end{align*}
% $$\norm{\hat{\Theta}^{22} - \Theta^{22}}_F \leq   O(\sqrt{n\rho})F_2\nu (1+\alpha_0)/n + O(n\rho)\{\Delta_2 F_2^2F_1+ 2F_2((\Delta_1^2 + 2\sqrt{n} \Delta_1)F_1^2)\}.$$


% we have
% \begin{equation*}
%     \mathbb{E}(||Q_1||_F^2)=\sum_{i,j}\text{Var}(Q_{1ij})\sim \rho n\text{tr}(HH^T)
% \end{equation*}
% and we know
% \begin{equation*}
%     \begin{aligned}
%         \text{tr}(HH^T) &= \text{tr}({B}^{-1}({\Theta}^{11T}{\Theta}^{11})^{-1}{\Theta}^{11T}{\Theta}^{11}({\Theta}^{11T}{\Theta}^{11})^{-1}{B}^{-1})\\
%         &= \text{tr}(B^{-1}({\Theta}^{11T}{\Theta}^{11})^{-1}{B}^{-1})\\
%         &= \text{tr}(({\Theta}^{11T}{\Theta}^{11})^{-1}{(BB)}^{-1})\\
%         &\leq ||({\Theta}^{11T}{\Theta}^{11})^{-1}||_{op}\text{tr}((BB)^{-1})\\
%         &\leq \frac{2\nu (1+\alpha_0)}{n}O(\frac{r}{\rho^2}),
%     \end{aligned}
% \end{equation*}
% so we have $\mathbb{E}(||Q_1||_F^2)\sim \rho n\frac{r}{n\rho^2}$. 

%For $Q_3$, we have
%\begin{equation*}
%\begin{aligned}
%    ||Q_3||_F^2 &= \text{tr}((\hat{H}-H)(\hat{H}-H)P^{12}P^{12})\\
    %&\leq  ||P^{12}P^{12}||_{op} \text{tr}((\hat{H}-H)(\hat{H}-H))\\
    %&= ||P^{12}P^{12}||_{op}(\tr{\hat{H}\hat{H}^T}+\tr{{H}{H^T}})
%\end{aligned}
%\end{equation*}
%(because the order of $H$ is $\rho^{-1}$).
\end{proof}

\begin{Proposition}
\label{prop:estmmsb}
Given the correct number of clusters $r$, then with high probability, $\langle A^{22},\hat{X}_{r}^{22} \rangle > \langle A^{22},X_0^{22} \rangle -O((n\rho)^{3/2}(\log n)^{1+\xi}).$

\end{Proposition}

\begin{proof}
First note
\begin{align}
    |\langle (A^{22})^2-\text{diag}((A^{22})^2),\hat{X}_{r}^{22}- {X}_0^{22}\rangle| & \leq |\langle \hat{S}^{22}-S^{22},\hat{X}_{r}^{22}- {X}_0^{22}\rangle|  \notag\\
    & \quad + |\langle S^{22},\hat{X}_{r}^{22}- {X}_0^{22}\rangle|,
    \label{eq:A2_estX}
\end{align}
where $\hat{S}^{22} = (A^{22})^2-\text{diag}((A^{22})^2)$, $S^{22}=(P^{22})^2-\text{diag}((P^{22})^2)$.

Consider SVD of $\hat{\Theta}^{22} = \hat{U}\hat{D} \hat{V}^T$ and $\Theta^{22} = U D V^T,$ then $\hat{X}_{r}^{22} = \hat{U}\hat{U}^T$, and $X_0^{22} = UU^T.$ For any orthogonal matrix $O$,
\begin{align}
    \norm{\hat{X}_{r}^{22}- {X}_0^{22}}_F &= \norm{\hat{U}\hat{U}^T - UU^T}_F = \norm{\hat{U}\hat{U}^T - UO(UO)^T}_F\notag\\
    &\leq \norm{(\hat{U}-UO)(\hat{U}-UO)^T}_F + 2 \norm{(\hat{U}-UO)(UO)^T}_F\notag\\
    &\leq \norm{\hat{U}-UO}_F^2 + 2 \norm{\hat{U}-UO}_F
    \label{eq:x_error}
\end{align}
Using the Theorem 2 in \cite{davis-kahan}, we know there exists $O$ such that, 

$$\norm{\hat{U}- UO}_F \leq \frac{2\norm{\hat{\Theta}^{22} - \Theta^{22}}_F}{\lambda_{r}(\Theta^{22})},$$
where $\lambda_{r}(\Theta^{22})$ is the $r$-th largest singular value of $\Theta^{22}$. Using Lemma 3.6 in \cite{Mao2017EstimatingMM}, w.h.p, $\lambda_{r_0}(\Theta^{22}) =\Omega(\sqrt{n}).$ Now by Lemma~\ref{lem:theta_est_error} and Eq~\eqref{eq:x_error}, w.h.p.
$$\norm{\hat{X}_{r_0}^{22}- {X}_0^{22}}_F = O(\frac{(\log n)^{1+\xi}}{\sqrt{n\rho}}).$$

Now in Eq~\eqref{eq:A2_estX}, 
$$
|\langle S^{22},\hat{X}_{r}^{22}- {X}_0^{22}\rangle| \leq \norm{S^{22}}_F \norm{\hat{X}_{r}^{22}- {X}_0^{22}}_F = O_P((n\rho)^{3/2}(\log n)^{1+\xi}),
$$
and
$$
|\langle \hat{S}^{22}-S^{22},\hat{X}_{r}^{22}- {X}_0^{22}\rangle| = O_P(n\rho\sqrt{log n})
$$
by Lemma~\ref{lem:A2_conc}.
\end{proof}

Finally we prove Theorem~\ref{thm:nok_mmsb}.

\begin{proof}[Proof of Theorem~\ref{thm:nok_mmsb}]
By Propositions~\ref{prop:underestimatemmsb}, \ref{prop:overestimatemmsb} and \ref{prop:estmmsb}, 
\begin{align*}
   \epsilon_{\text{under}} & = \Omega(n^2\rho^2),  \\ 
   \epsilon_{\text{est}} & = O((n\rho)^{3/2}(\log n)^{1+\xi}),    \\
   \epsilon_{\text{over}} &= O(n\rho\sqrt{\log n}).
\end{align*}
Then the result follows by setting $\Delta=O((n\rho)^{3/2}(\log n)^{1+\xi})$.
\end{proof} 


%Now throw away all constants other than $n$ and $\rho$ (treat $r_0$, $\nu$,  $\alpha_0$, $\lambda^*(B_0)$ as costant), and assume $r_0^3 / \sqrt{n\rho} = o_P(1),$ 
%$$\norm{\hat{H} - H}_F\leq \tilde{O}(\frac{r_0^{4.5}}{n\rho ^{3/2}})$$

%$$\norm{\hat{\Theta}^{22} - \Theta^{22}}_F\leq \tilde{O}(\frac{r_0^{4.5}}{\rho ^{1/2}})$$

%$$\norm{\hat{U}- UO}_F\leq \tilde{O}(\frac{r_0^{4.5}}{\sqrt{n\rho}})$$

%$$\norm{\hat{X}_{r_0}^{22}- {X}_0^{22}}_F \leq \tilde{O}(\frac{r_0^{4.5}}{\sqrt{n\rho}})$$




\section{Detailed parameter settings in experiments and additional results}
\label{sec:expdetail}
\subsection*{Motivating examples in Section~\ref{sec:knownk} (Figure~\ref{fig:yd_motivation})} 

In Figure~\ref{fig:yd_motivation}(a)-(b), we generate an adjacency matrix from a SBM model with four communities, each having 50 nodes, and
$$B = \begin{bmatrix} 
0.8 & 0.6 & 0.4 & 0.4 \\
0.6 & 0.8 & 0.4 & 0.4 \\
0.4 & 0.4 & 0.8 & 0.6 \\
0.4 & 0.4 & 0.6 & 0.8 
\end{bmatrix}.$$

In Figure~\ref{fig:yd_motivation}(c)-(d), we consider a four-component Gaussian mixture model, where the means $\mu_1, \dots, \mu_4$ are generated from Gaussian distributions centered at $(0,0), (0,0), (5,5), (10,10)$ with covariance $6 I$, so that the first two clusters are closer to each other than the rest. Then we generate 1000 data points centered at these means with covariance $0.5 I$,  each point assigned to one of the four clusters independently with probability $(\frac{20}{42}, \frac{20}{42}, \frac{1}{42}, \frac{1}{42})$. Finally, we introduce correlation between the two dimensions by multiplying each point by $\begin{bmatrix} 
2 & 1 \\
1 & 2 
\end{bmatrix}$.

\begin{comment}
\subsection*{Tuning with \ref{SDP:YD} (Figure~\ref{fig:yd1})}
\textbf{Figure~\ref{fig:yd1} (a,b):} We first consider graphs generated from a hierarchical SBM  with equal sized clusters, where 
$$B = \text{sparsity}\times \begin{bmatrix} 
0.8 & 0.6 & 0.3 & 0.3 \\
0.6 & 0.8 & 0.3 & 0.3 \\
0.3 & 0.3 & 0.8 & 0.6 \\
0.3 & 0.3 & 0.6 & 0.8 
\end{bmatrix}.$$
Each cluster has 100 nodes and the sparsity constant ranges from $0.2$ to $1$.

\textbf{Figure~\ref{fig:yd1} (c,d):} Next, we consider graphs generated from a SBM with the same $B$ matrix, but with unequal cluster sizes. 
Cluster 1 and 3 have 100 nodes each, while cluster 2 and 4 have 50 nodes each. The sparsity constant ranges from $0.2$ to $1$.
\end{comment}

\subsection*{Tuning with spectral clustering (Figure~\ref{fig:sp2})}
 
We generate the means $\mu_a, a\in[3]$ from $d=20$ dimensional Gaussian distribution with covariance $0.01I$. To impose sparsity on each $\mu_{a}$, we set all but the first two dimensions to 0.  To change the level of clustering difficulty, we multiply $\mu_a$ with a separation constant $c$, and a larger $c$ leads to larger separation and easier clustering. We vary $c$ from $0$ to $200$. We generate $n=500$ samples from each mixture with a constant covariance matrix (an identity matrix) using Eq~\ref{eq:mog}.  For Figure~\ref{fig:sp2} (a,b), the probabilities of cluster assignment are equal, while for  Figure~\ref{fig:sp2} (c,d), each point belongs to one of the three clusters with probability $(\frac{20}{22}, \frac{1}{22}, \frac{1}{22})$. 

\subsection*{Additional figure for Section~\ref{sec:exp_matr_mixture}}

\begin{figure}[h]
\begin{subfigure}[t]{.33\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{NIPS2019_UL/figures/results/true_mnist_scatter.png}
  %\hspace{-2em}\includegraphics[width=1\linewidth]{figures/figures_purna/balanced_cluster_scatter.jpg}
  \vspace{-5mm}
  \caption{True clustering}
\end{subfigure}\hspace{-3mm}
\begin{subfigure}[t]{.33\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{NIPS2019_UL/figures/results/matr_mnist_scatter.png}
  %\hspace{-2em}\includegraphics[width=1\linewidth]{figures/figures_purna/balanced_cluster_scatter.jpg}
  \vspace{-5mm}
  \caption{Clustering by MATR}
\end{subfigure}\hspace{-3mm}
\begin{subfigure}[t]{.33\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{NIPS2019_UL/figures/results/ds_mnist_scatter.png} 
 %\includegraphics[width=1\linewidth]{figures/figures_purna/balanced_clustering_nmi.jpg} 
  \vspace{-5mm}
  \caption{Clustering by DS}
\end{subfigure}\hspace{-3mm}\\
\centering
\begin{subfigure}[t]{.33\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{NIPS2019_UL/figures/results/knn_mnist_scatter.png}
  \vspace{-5mm}
  \caption{Clustering by KNN}
\end{subfigure}\hspace{-3mm}
\begin{subfigure}[t]{.33\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{NIPS2019_UL/figures/results/mst_mnist_scatter.png}
  \vspace{-5mm}
   \caption{Clustering by MST}
\end{subfigure}%
\caption{Visualization of clustering results on handwritten digits dataset.}
\label{fig:tsne}\vspace{-3mm}
\end{figure}

\subsection*{Tuning with \ref{SDP:BW} (Figure~\ref{fig:matr-cv})}
\textbf{Figure~\ref{fig:matr-cv} (a):} We first consider graphs generated from a SBM with equal sized clusters, where 
$$B = \rho\times \begin{bmatrix} 
0.8 & 0.5 & 0.3 & 0.3 \\
0.5 & 0.8 & 0.3 & 0.3 \\
0.3 & 0.3 & 0.8 & 0.5 \\
0.3 & 0.3 & 0.5 & 0.8 
\end{bmatrix}.$$
Each cluster has $100$ nodes and $5$ $\rho$'s are selected from $0.2$ to $0.6$ with even spacing.

\textbf{Figure~\ref{fig:matr-cv} (b):} Here we consider graphs generated from an unequal-sized SBM , where the $B$ matrix is the same as above. The clusters have $120,80,120,80$ nodes respectively. The same $\rho$'s as above are used.


\textbf{Table~\ref{tab:MATR_CV_K} (a,b):} We show the median number of clusters selected by each method as $\rho$ changes. The ground truth is 4 clusters.

% \begin{table}[]
% \begin{subtable}[t]{0.50\textwidth}
% \centering
% \begin{tabular}[t]{|l|l|l|l|}
% \hline
%      & MATR-CV & BH   & ECV \\
% \hline       
% 37.77  & 0     & 0  & 0 \\
% \hline
% 56.61  & 0     & 0  & 0\\
% \hline
% 75.65  & 4    & 0  & 0 \\
% \hline
% 94.94  & 3   & 0  & 0 \\
% \hline
% 113.62 & 5   & 3 & 2 \\
% \hline
% \end{tabular}
% \caption{Exact recovery times for equal size case out of $5$ random graphs}
% \end{subtable}%
% \begin{subtable}[t]{0.50\textwidth}
% \centering
% \begin{tabular}[t]{|l|l|l|l|}
% \hline
%       & MATR-CV & BH   & ECV \\
% \hline       
% 38.10  & 0     & 0  & 0 \\
% \hline
% 57.30  & 0     & 0  & 0\\
% \hline
% 76.41  & 0    & 0  & 0 \\
% \hline
% 95.55  & 4    & 0 & 0 \\
% \hline
% 114.04 & 3   & 0 & 2 \\
% \hline
% \end{tabular}
% \caption{Exact recovery times for unequal size case out of $5$ random graphs}
% \end{subtable}%
% \caption{Comparison of exact recovery number along with average degree for all algorithms.}
% \label{tab:MATR_CV_K}
% \end{table}

\begin{table}[]
\begin{subtable}[t]{0.50\textwidth}
\centering
\begin{tabular}[t]{|l|l|l|l|}
\hline
  $\rho$   & MATR-CV & BH   & ECV \\
\hline       
0.2  & 2     & 2  & 2 \\
\hline
0.3  & 2     & 2  & 2\\
\hline
0.4  & 4    & 2  & 2 \\
\hline
0.5  & 4   & 2  & 2 \\
\hline
0.6 & 4   & 4 & 2 \\
\hline
\end{tabular}
\caption{Median number of clusters selected for equal size case out of $5$ random graphs}
\end{subtable}%
\begin{subtable}[t]{0.50\textwidth}
\centering
\begin{tabular}[t]{|l|l|l|l|}
\hline
  $\rho$    & MATR-CV & BH   & ECV \\
\hline       
0.2  & 2     & 2  & 2 \\
\hline
0.3  & 2     & 2  & 2\\
\hline
0.4  & 3    & 2  & 2 \\
\hline
0.5  & 4    & 2 & 2 \\
\hline
0.6 & 4   & 3 & 2 \\
\hline
\end{tabular}
\caption{Median number of clusters selected for unequal size case out of $5$ random graphs}
\end{subtable}%
\caption{Comparison of model selection results along with $\rho$ for all algorithms.}
\label{tab:MATR_CV_K}
\end{table}


\bibliographystyle{plainnat}
\bibliography{reference.bib}
\end{document}
